Debugging and Runtime Analysis of Neural Networks with VLMs (A Case Study)

Debugging of Deep Neural Networks (DNNs), particularly vision models, is very challenging due to the complex and opaque decision-making processes in these networks. In this paper, we explore multi-modal Vision-Language Models (VLMs), such as CLIP, to automatically interpret the opaque representation space of vision models using natural language. This in turn, enables a semantic analysis of model behavior using human-understandable concepts, without requiring costly human annotations. Key to our approach is the notion of semantic heatmap, that succinctly captures the statistical properties of DNNs in terms of the concepts discovered with the VLM and that are computed off-line using a held-out data set. We show the utility of semantic heatmaps for fault localization -- an essential step in debugging -- in vision models. Our proposed technique helps localize the fault in the network (encoder vs head) and also highlights the responsible high-level concepts, by leveraging novel differential heatmaps, which summarize the semantic differences between the correct and incorrect behaviour of the analyzed DNN. We further propose a lightweight runtime analysis to detect and filter-out defects at runtime, thus improving the reliability of the analyzed DNNs. The runtime analysis works by measuring and comparing the similarity between the heatmap computed for a new (unseen) input and the heatmaps computed a-priori for correct vs incorrect DNN behavior. We consider two types of defects: misclassifications and vulnerabilities to adversarial attacks. We demonstrate the debugging and runtime analysis on a case study involving a complex ResNet-based classifier trained on the RIVAL10 dataset.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

ACMCPSAMPLES= \
	samples/sample-acmcp-Discussion.pdf \
	samples/sample-acmcp-Invited.pdf \
	samples/sample-acmcp-Position.pdf \
	samples/sample-acmcp-Research.pdf \
	samples/sample-acmcp-Review.pdf \

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-sigconf-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*

acmcp.zip: ${ACMCPSAMPLES} acmart.cls
	zip $@ $+

samples/sample-acmcp.tex: samples/samples.ins samples/samples.dtx
	cd samples; pdflatex samples.ins; cd ..


samples/sample-acmcp-%.tex: samples/sample-acmcp.tex samples/acm-jdslogo.png
	sed 's/acmArticleType{Review}/acmArticleType{$*}/' $< > $@

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 2.03.  Cleaned generation of samples.
	       New options for printing conference proceedings
	       in ACM journals

Version 2.02   Documentation update.
	       Changes in TOG templates
	       Corrected typo in ACM/IMS journals

Version 2.01   \acmPrice now produces a warning.

Version 2.00   ACM switches to electronic only version.
	       We do not print article tabs anymore.
	       New copyright wording.
	       Deleted \acmPrice.

Version 1.93   Added PACMSE

Version 1.92   Documentation update
	       Emergency change: changed order of hyperref and hyperxmp
	       due to changes in the undelying packages

Version 1.91   Minor changes in ACMCP format

Version 1.90a  Changes in the sample keywords and concepts

Version 1.90   Journal ISSN updated

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> abstract_new.tex <==
Debugging, testing, and runtime monitoring of Deep Neural Network (DNN) models, particularly vision models, are challenging due to their complex and opaque decision-making processes. 
%Typically, the early layers of DNNs, specifically vision models, extract and represent semantic information, e.g., concepts. 
Multi-modal Vision-Language Models (VLMs) such as CLIP offer an exciting opportunity to interpret the representation space of vision models using natural language. This allows analysis of model behavior using human-understandable concepts, such as ``wheels". In this paper, leveraging concept-based analysis through VLMs, we propose a statistical approach to analyzing DNN behavior by summarizing and visualizing concepts as heatmaps. \divya{added this.} We show the utility of the concept-based heatmaps for offline analysis; explaining behavior, debugging, and examination of feature robustness, as well as runtime detection of adversarial inputs. 
%We demonstrate that our method is effective for explaining behavior, debugging, robustness analysis, and runtime detection of adversarial inputs. 
Our approach provides valuable insights into model behavior, and thus guides the development of more effective and interpretable analysis of DNNs. \susmit{Our title is a bit too generic. Should we focus on semantic heatmaps and have a title around that, say, ``Offline analysis and runtime monitoring of DNNs using Semantic Heatmaps"? We could then say, the primary contribution of this paper is concept-based heatmaps and we show its utility for offline/online assurance.} \divya{Please let us know your opinion on the current title and abstract.}

==> figures/workflow.tex <==
\tikzstyle{roundbox} = [rectangle, rounded corners, 
minimum width=1.3cm, 
%minimum height=1cm,
text centered, 
draw=black, 
fill=white!30]


\tikzstyle{roundboxconcepts} = [rectangle,
%minimum width=3cm, 
%minimum height=1cm,
text width=1.3cm, 
text centered, 
draw=black, 
fill=gray!30]

\tikzstyle{roundboxtext} = [rectangle, rounded corners, 
minimum width=2cm, 
minimum height=0.7cm,
text centered, 
draw=black, 
fill=white!30]

\tikzstyle{roundboximage} = [rectangle, rounded corners, 
minimum width=2cm, 
minimum height=0.7cm,
text centered, 
draw=black, 
fill=white!30]


\tikzstyle{emb} = [rectangle, rounded corners, 
minimum width=1.2cm, 
minimum height=0.5cm,
text centered, 
draw=black, 
text width=0.8cm, 
fill=white!30]


\tikzstyle{roundboxhead} = [rectangle, rounded corners, 
minimum width=1.5cm, 
%minimum height=1cm,
text centered, 
draw=black, 
fill=white!30]


\tikzstyle{mapper} = [trapezium, 
%trapezium stretches=true, % A later addition
trapezium left angle=-110, 
trapezium right angle=70, 
minimum width=0.5cm, 
%minimum height=1cm, 
text centered, 
draw=black, fill=gray!30]

\tikzstyle{modelclip} = [rectangle, , rounded corners, 
minimum width=8cm, 
minimum height=2cm, 
text centered, 
text width=3cm, 
draw=white, 
fill=orange!30]

\tikzstyle{modelmodel} = [rectangle, , rounded corners, 
minimum width=8cm, 
minimum height=1.3cm, 
text centered, 
text width=3cm, 
draw=white, 
fill=green!20]

\tikzstyle{concepts} = [rectangle,  rounded corners, 
minimum width=4cm, 
minimum height=2cm, 
text centered, 
text width=3cm, 
draw=white, 
fill=pink!30]

\tikzstyle{decision} = [diamond, 
minimum width=3cm, 
minimum height=1cm, 
text centered, 
draw=black, 
fill=green!30]
\tikzstyle{arrowgray} = [very thick,gray,->,>=stealth]
\tikzstyle{arrow} = [ thick,->,>=stealth]
\tikzstyle{arrowdashed} = [ thick,->,dashed,>=stealth]
\tikzstyle{line}     = [ thick,draw, -latex']


\begin {figure*}%[!hbtp]
\centering
\begin{tikzpicture}[node distance=2cm]
\node (concepts) [roundboxconcepts,  font=\small] {classes, concepts};
\node (start) [roundbox,  below of=concepts, yshift=0.5cm, font=\small] {Images};
\node (cliptext) [roundboxtext, right of=start, xshift=1.2cm, yshift=1cm, font=\small] {$\encode{g}^{txt}$};
\node (clipimage) [roundboximage, right of=start, xshift=1.2cm, font=\small] {$\encode{g}^{img}$};
\node (image) [roundboximage, right of=start, xshift=1.2cm, yshift=-2.4cm, font=\small] {$\encode{f}$};
\node (clipemb) [emb, right of=cliptext, xshift=1.3cm, yshift=-0.5cm, rotate=90, font=\small] {embs};
\node (imageemb) [emb, right of=image, xshift=1.3cm, yshift=0cm, rotate=90, font=\small] {embs};
\node (map) [mapper, above of=imageemb, xshift=-0cm, yshift=-0.6cm, rotate=90, font=\small] {$\repmap$};
\node (imagehead) [roundboxhead, right of=imageemb, font=\small] {$\head{f}$};
\node (cliphead) [roundboxhead, right of=clipemb, yshift=-0.5cm, font=\small] {$\cosine$ similarity};
\node (conceptsemb) [roundboxconcepts, above of=clipemb, font=\small] {Embeddings  $\condir{con_i}$};
\node (heat) [roundboxhead, right of=clipemb, xshift=2.9cm,  yshift=0cm, font=\small] {heatmaps};



%\node (pro1) [process, below of=in1] {Process 1};
%\node (dec1) [decision, below of=pro1, yshift=-0.5cm] {Decision 1};

% \node (pro2a) [process, below of=dec1, yshift=-0.5cm] {Process 2a
% text text text text
% text text text 
% text text text};

% \node (pro2b) [process, right of=dec1, xshift=2cm] {Process 2b};
% \node (out1) [io, below of=pro2a] {Output};
% \node (stop) [startstop, below of=out1] {Stop};

%\draw [arrow] (start) -- (cliptext);
\draw [arrow] (start) -- (clipimage);
\draw [arrow] (start) -- (image);
\draw [arrow] (image) -- (imageemb);
\draw [arrow] (imageemb) -- (imagehead);
\draw [arrow] (imageemb) -- (map);
\draw [arrow] (map) -- (clipemb);
\draw [arrowgray] (concepts) --  (cliptext);
\draw [arrowgray] (cliptext) -- ([yshift=-2mm]clipemb.north east);
\draw [arrow] (clipimage) -- ([yshift=2mm]clipemb.north west);
\draw [arrow] ([yshift=1mm]clipemb.south west) -- (cliphead);
\draw [arrow] (clipemb) --  (heat);
\draw [arrowgray] (clipemb) -- (conceptsemb);

\path[line] (conceptsemb.east) -- +(0,0) -|  (heat.north) node[pos=0.25,above]{} ;  


% \draw [arrow] (in1) -- (pro1);
% \draw [arrow] (pro1) -- (dec1);
% \draw [arrow] (dec1) -- node[anchor=east] {yes} (pro2a);
% \draw [arrow] (dec1) -- node[anchor=south] {no} (pro2b);
% \draw [arrow] (pro2b) |- (pro1);
% \draw [arrow] (pro2a) -- (out1);
% \draw [arrow] (out1) -- (stop);
  \begin{scope}[on background layer]
    \node [modelclip,above left=3mm of cliptext, anchor=north west, text width=2cm,label={[anchor=north east]north east:Multi-modal $g$ (CLIP)}] (clip) {};
  %you may also use align = center instead of text width = ...
  \end{scope}

\begin{scope}[on background layer]
    \node [modelmodel,above left=3mm of image,yshift=0.1cm,  anchor=north west, text width=2cm, label={[anchor=north east]north east:Model $f$}] (model) {};
  %you may also use align = center instead of text width = ...
  \end{scope}

\begin{scope}[on background layer]
    \node [concepts,right=1mm of clip, anchor=north west, text width=2cm, yshift=1cm,  label={[anchor=north east]north east:Concepts analysis}] (cons) {};
  %you may also use align = center instead of text width = ...
  \end{scope}

\path (start) edge [bend left=15, blue!50,very  thick,dashed] (image);
\path (image) edge [bend left=15, blue!50,very  thick,dashed] (imageemb);
\path (imageemb) edge [bend left=15, blue!50,very  thick,dashed] (map);
\path (map) edge [bend left=15, blue!50,very  thick,dashed] ([yshift=1mm]clipemb.north west);
\path (clipemb) edge [bend left=15, blue!50,very  thick,dashed] ([yshift=-1mm]heat.north west);

  
\end{tikzpicture}
\caption{\label{fig:flow}The diagram shows the workflow of our approach. The offline phase is represented with gray boxes and arrows, where we precompute the $\repmap$ and the embeddings of relevant concepts and classes. The blue path illustrates the online phase, showing how the image is processed through the image encoder and a linear map to obtain its embedding in the representation space of VLM.\caroline{could we also show $g_{head}$ somewhere in here?}\nina{sure, should I replace cos similarity with $g_{head}?$ or just add another box}\caroline{maybe just another box?}\susmit{Too much free/white space - we could increase font and reduce white space.}\nina{This diagram is work in progress for now. We might add other blocks. After that, I will make it look nicer.}}
\end{figure*}

==> sections/applications_copy.tex <==
\section{Analysis Results}

\subsection{Application 1: Explaining Correct Behavior}
\label{subsec:explain_beh}
%\caroline{summary of this paragraph: heatmaps help visualize whether outputs are produced for the right reasons.}
%\corina{do we explain anywhere why explaining correct behaviour is useful? perhaps in intro?}
Given inputs that are correctly classified by the vision model, i.e., model output matches the ground truth, 
%Given a set of inputs on which the model produces outputs matching the ideal label, 
we aim to understand if the model produces these outputs for the \textit{right reasons}, which helps build trust in the behavior of the model beyond testing. Using our semantic heatmaps, we can visualize concepts utilized by the model for producing these outputs. 

We use images and concepts related to class \textit{truck} to illustrate our ideas.
Fig.~\ref{sfig:correct_truck} 
%To visualize concepts in inputs that led to the output \textit{truck} by ResNet18, in Fig.~\ref{sfig:correct_truck}, 
%we show the summary heatmap constructed with all \textit{truck} images from the RIVAL10 test set correctly classified by ResNet18.
%we show the
depicts the ground-truth summary heatmap computed with all \textit{truck} images from the RIVAL10 test set that are correctly classified by ResNet18. %\ravi{made minor edit, please check}
%\ravi{This kind of summary heatmap is not convered under any of the three different kinds we disucssed in the previous section. Should we merge ground truth based and output label based?}
From the heatmap, we see that ResNet18 can satisfy most relevant predicates, i.e., the ones involving concepts relevant to \textit{trucks} (highlighted with red outlines) with high probability, 
%satisfaction probability of relevant concepts (highlighted with red outlines) 
except for the predicate $metallic>tail$, and predicates involving concept \textit{text}, e.g., $text>tail$ and $text>horns$. 
%This suggests that ResNet18 can indeed identify objects that are \textit{long, rectangular, tall,} and \textit{metallic} with \textit{wheels} as \textit{trucks}; but struggles to effectively identify text in images, and distinguish \textit{metallic} and \textit{tails}. \ravi{From Fig 3b, we can only draw conclusion about model behavior on trucks, so this sentence seems too strong. }
This suggests that when ResNet18 correctly classifies images as \textit{trucks}, it indeed does so for the \emph{right reasons}---it is able to recognize the strong presence of concepts such as \textit{long, rectangular, tall, metallic} with \textit{wheels} in these images. However the model struggles to effectively identify text in images, and distinguish \textit{metallic} and \textit{tails}.
Such information can facilitate performance improvements of the vision models, e.g., guiding data selection for retraining. Additionally, notice that some non-relevant predicates also have high satisfaction probabilities, e.g., $tail>beak$. This could be the result of other concepts in the images, the dependency between relevant and non-relevant concepts, or how the CLIP model is trained. Further analysis is required to determine the cause, we leave this as future work.

Fig.~\ref{fig:all_truck} shows the ground-truth summary heatmap of all images with ground-truth \textit{truck}. It is visually similar to the summary heatmap of all images correctly classified as \textit{truck} ((Fig.~\ref{sfig:correct_truck})) with most relevant strength predicates for \textit{trucks} satisfied with a high probability.  
%This suggests that ResNet18 is able to correctly encode relevant concepts in its representation space for the majority of in-distribution inputs, and this is expected due to the high accuracy of ResNet18 on these images.
%\ravi{Not very clear. Fig 3a shows us that for images with ground truth truck, model is able to correctly identify the relevant strength predicates, indicating that it is able to correctly encode relevant concepts in its representation space for the majority of in-distribution truck inputs. Given Fig 3b is very similar to Fig 3a, it further shows that when the model predicts truck correctly, it does so for the right reasons. The analysis in previous para also shows this.} 
This suggests that ResNet18 is able to correctly extract the relevant concepts  for the majority of \textit{truck} inputs, and this is expected due to the high accuracy of ResNet18 on these images.
However, in the following sections, as we delve deeper into the representation space for subsets of inputs that are incorrectly classified, we discover that the encoder incorrectly encodes a subset of inputs which leads to misclassification. 
%\susmit{A bit confusing sentence - was the incorrect encoding only for incorrectly classified inputs? If so, remove ``correctly and".}\caroline{addressed, removed ``correctly and"}

%\caroline{future directions? interpretation, data selection, finetuning?}


%{\it Heatmap for correctly classified inputs for Rival10. \blue{added, see Fig.~\ref{fig:correct_truck}}\it} 

\begin{figure*}[t]
    \centering
    \begin{subfigure}{0.23\linewidth}
        \centering
        \includegraphics[width=\linewidth]{heatmaps/resnet/all_GT_truck.jpg}
    %\vspace{-0.25in}
    \caption{With all images with ground truth \textit{truck}.}
    \label{fig:all_truck}
    \end{subfigure}
    \hspace{0.05in}
    \begin{subfigure}{0.23\linewidth}
        \centering
        \includegraphics[width=\linewidth]{heatmaps/resnet/all_correct_truck.jpg}
        \vspace{-0.25in}
        \caption{With images correctly classified as \textit{truck}. }
        \label{sfig:correct_truck}
    \end{subfigure}
    \hspace{0.05in}
    \begin{subfigure}{0.23\linewidth}
        \centering
        \includegraphics[width=\linewidth]{heatmaps/resnet/all_GT_enc_error_truck.jpg}
        \vspace{-0.25in}
        \caption{With misclassified \textit{truck} images due to encoder error.}
        \label{sfig:truck_enc}
    \end{subfigure}
    \hspace{0.05in}
    \begin{subfigure}{0.23\linewidth}
        \centering
        \includegraphics[width=\linewidth]{heatmaps/resnet/all_GT_head_error_truck.jpg}
        \vspace{-0.25in}
        \caption{With misclassified \textit{truck} images due to head error.}
        \label{sfig:truck_head}
    \end{subfigure}
    \vspace{-0.1in}
    \caption{Ground-truth summary heatmaps for images with ground truth \textit{truck}. The red outline indicates relevant strength predicates for class \textit{truck}. }
    \label{fig:resnet-error}
    \vspace{-0.15in}
\end{figure*} 


\subsection{Application 2: Debugging}
\label{subsec:debugging}

\begin{figure*}
\centering
\includegraphics[scale=0.35]{figures/ENC_HEAD_ERR_examples.png}
%\caption{Examples of misclassified inputs for ResNet18 model, localized to bug in the encoder (Encoder Error) and bug in the head (Head Error).}
\vspace{-0.1in}
\caption{Examples of misclassified inputs of ResNet18, error localized to the encoder (Encoder Error) and the head (Head Error).}
\label{fig:enc_head_errs}
\label{fig:enc_head_errs}
\end{figure*}

For inputs that are misclassified by the vision model, i.e., the model output does not match the ground truth, 
%Given a set of inputs on which the model fails, 
we wish to investigate the cause of failures, which can further aid in activities such as targeted testing and repair.%, and re-training to improve the model performance. 

%We investigate the following types of failures; mis-classified in-distribution inputs and inputs with specific types of perturbations. (this is probably not this application)
%{\it How does CLIP perform when fed directly with perturbed inputs? \it} 

%\paragraph{Setup} 
%\begin{itemize}
%    \item Dataset: Rival10
%    \item vision models: Resnet18, Resnet50, vit\_tiny, VLM: clip
%    \item t2c mappings
%    \item perturbations: adversarial, poison, natural (brightness, noise, etc.)
%\end{itemize}

\subsubsection{Localization to Encoder and Head Errors}
%\subsubsection{Encoder and Head Errors} %\caroline{summary of this paragraph: def of encoder vs head error.}
Consider an input $x$ with ground truth $c_0 \in C$ such that $f(x)\neq c_0$, i.e., misclassified by the vision model. The decomposition of the vision model into an image encoder $f_{enc}$ and a classification head $f_{head}$ (see Sec.~\ref{sec:overview}) allows us to localize errors to a specific part of the model. The misclassification can be caused by errors in the encoder, i.e., the encoder does not correctly encode relevant concepts; or errors in the head, i.e., concepts are encoded correctly but the wrong output label is produced; or both. The location of the error can be detected through strength predicates. Intuitively, if the strength predicates relevant for the ground truth label of $x$ are not satisfied by its image embedding, then the encoder has incorrectly encoded the image; otherwise, the error is in the head. %Note that with encoder errors, errors in the head may be present at the same time. However, since updating the encoder would also affect the head, the encoder errors should be addressed first, thus we consider such a case as encoder errors. 
Note that, for an image $x$, encoder and head errors may be present at the same time. However, since updating the encoder would also require updating the head, the encoder errors should be addressed first, thus we consider such cases as exclusively encoder errors. %\ravi{reworded slightly; check}
We present an %\divya{perhaps remove lighweight since we do not show that it is lightweight?}\caroline{removed} 
approach to localize errors as encoder or head errors, and then use summary semantic heatmaps to validate the localization and analyze the errors.


%As explained in section~\ref{sec:overview}, this could be caused due to an error in the encoder (does not encode relevant features correctly), or an error in the head (does encode the features correctly, but the classification head does not apply the correct logic for classification), or in both. 
%Our insight is that if there is a problem in the encoder, then the representation space should highlight this (i.e) the embedding vector corresponding to the misclassified input would not satisfy relevant strength predicates for the GT label. If the embedding vector does satisfy the relevant strength predicates, then the problem could be isolated to the head. 
%Note that, in the former case, the problem could also be in the head but we consider them as {\it encoder \it} errors, since we know for sure that there are problems in the encoder that could be addressed first.
%We could adopt the above-mentioned technique and evaluate single-input heatmaps of every misclassified input. However, every input may satisfy a different set of relevant (and) irrelevant strength predicates, which may can complicate the analysis. We present a lightweight approach to first categorize encoder and head errors, and then use summary concept heatmaps to validate the localization.

%Intuitively, if an embedding vector does not satisfy a sufficient number of strength predicates for a label, then a zero-shot classification via $g_{head}$ would not give the correct label.
%\ravi{Not sure I understand. What is embedding vector referring to here? Is it it embedding generated $f_{enc}$ or $g_{enc}$?}
%\divya{should we define formally or explain how zero-shot classification via $g_{head}$ is done?}\caroline{I think this is in background} \corina{yes it is explained in background} \divya{Since here we present an algorithm for localization using zero-shot classification, I was thinking if we should give more details or formalize $g_{head}$.} 
 
%\divya{We could directly use concept heatmap for an input to  categorize it as encoder error vs head error. Should we give some reason why we choose to use zero-shot classification instead?} \caroline{I guess the reason would be: we kind of use the VLM as the oracle in this paper, this would give us the most precise results?} 
%
%Therefore, %\caroline{assuming VLM correct added here}consider an input $x$ with ground truth $c_0$ that the VLM correctly classifies, i.e., $g_{head}(g_{enc}^{img} (x)) = c_0$ but the model misclassifies, i.e., $f(x) \neq c_0$.  
%However, to use this approach, we need to ensure that $g_{head}$  is accurate. We validate the zero-shot classification of CLIP for all test inputs (mis-classified by ResNet18); $e1 = g^{img}_{enc}(x) ; c = g_{head}(e1); c = c_{0}$ . We found the accuracy to be very high (TBD). <- I don't think we need this, we said the acc of CLIP earlier. 
%Therefore, for every input, we can then check if $e2 = r_{map}(x) ; g_{head}(e2)$ gives the correct label, or more simply if $g_{head}(e1) = g_{head}(e2)$. Subsequently, we categorize mis-classified inputs where $g_{head}(e1) \ne g_{head}(e2)$ as {\it encoder errors \it}, and  {\it head errors \it} otherwise. 
%Our concept-based analysis assumed that vision models can be decomposed into an image encoder $f_{enc}$ and a classification head $f_{head}$. This decomposition, together with the mapping from the vision model to the VLM, allows us to localize errors to a specific part of the model, i.e., encoder or head, that needs to be repaired or fine-tuned. %We can distinguish between encoder and head errors through the mapping from the vision model to the VLM. 
%Consider an input $x$ with ground truth $c_0 \in C$ such that $f(x)\neq c_0$, i.e., misclassified by the vision model, and $g(x) = c_0$, i.e., correctly classified by the VLM. 
%Intuitively, we consider the misclassification caused by errors in the encoder $f_{enc}$ if the embedding of this image does not correspond to the actual features in the image, e.g., wheels in the image incorrectly mapped to the embedding space of beaks.


Consider an input $x$ with ground truth $c_0$ that the VLM correctly classifies, i.e., $g_{head}(g_{enc}^{img} (x)) = c_0$ but the model misclassifies, i.e., $f(x) \neq c_0$.
Let $e_1 := r_{map}(f_{enc}(x))$ refer to the embedding of $x$ produced by the vision model, and let $e_2:= g^{img}_{enc}(x)$ refer to the embedding of $x$ directly produced by the VLM. 

\vspace{0.05in}
\noindent{\textit{\textbf{Localizing Encoder Error.}}}
If $e_1$ and $e_2$ lead to different zero-shot classification outputs, i.e., $g_{head}(e_1) \neq g_{head}(e_2)$, then we can localize that the error is in $f_{enc}$, we call it \textit{encoder error}. 
%\divya{should we mention we assume $g_{head}(e2)$ is correct?}\caroline{added}. 
%\end{definition}

\vspace{0.05in}
%\begin{definition}[Head Error]
\noindent{\textit{\textbf{Localizing Head Error.}}}
%Otherwise, $g_{head}(e_1) = g_{head}(e_2) = c_0 \neq f(x)$, suggesting that the embedding computed by $f_{enc}$ and mapped to the VLM's representation space via $r_{map}$ allows the VLM head to output the correct label, thus the error is in $f_{head}$; we call it \textit{head error}.
If $e_1$ and $e_2$ lead to the same zero-shot classification outputs, i.e., $g_{head}(e_1) = g_{head}(e_2)$, it suggests that the embedding computed by $f_{enc}$ and mapped to the VLM's representation space via $r_{map}$ allows the VLM head to output the correct label, thus the error is in $f_{head}$; we call it \textit{head error}.
%\end{definition}

For example, consider the \textit{ship} images on the left of Fig.~\ref{fig:enc_head_errs} that are mislcassified by ResNet18. The one on the left is misclassified due to the encoder error because $g_{head}(e_2)$ (i.e., CLIP) is \textit{ship} but $g_{head}(e_1)$ (i.e., CLIP via $r_{map}$) is \textit{frog}. 
The one on the right is misclassified due to the head error because $g_{head}(e_2)$ (i.e., CLIP) and $g_{head}(e_1)$ (i.e., CLIP via $r_{map}$) are both \textit{ship} but the ResNet18 output is \textit{dog}.
%\nina{If we have space, I would frame these as definitions (or highlighted somehow) as these are basic notions: encoder and head errors.}. %\caroline{added some sentences about Fig.~\ref{fig:enc_head_errs}} %\divya{maybe we could move these details to 4.3.2 , where we refer to Fig 4? }\caroline{I feel like these examples help with understanding the definition of encoder/head error}

By checking RIVAL-10 test images misclassified by ResNet18, we categorized 61 images as encoder errors (see Fig.~\ref{sfig:truck_enc} for the summary heatmap of misclassified \textit{truck} images) and 84 images as head errors (see Fig.~\ref{sfig:truck_head} for the summary heatmap for the summary heatmap of misclassified \textit{truck} images) respectively. Fig.~\ref{fig:enc_head_errs} shows examples of encoder and head errors identified by our technique. 

\subsubsection{Validating Localization with Mutations.} 
%\subsubsection{Error Localization} %\caroline{summary of this paragraph: we use a mutation-based approach to demonstrate encoder and head error. mutation in encoder [resp. head] led to a significant increase in No. encoder [resp. head] errors. Additionally, with an alternative decomposition, we can localize errors even more, e.g., with residual block 3. }

%\ravi{Section4.3.1 is also about error localization, so I renamed this subsubsection}

%Application of the above technique on the test inputs with ground-truth truck that are misclassified by ResNet18, we categorize 61 as encoder errors and 84 as head errors respectively.

%We would like to use ground-truth based summary heatmaps to validate this categorization. We expect that for inputs localized as encoder errors, the corresponding embedding vectors would not satisfy the strength predicates relevant to the ground-truth label, while the embedding vectors for the head errors would satisfy the relevant strength predicates.

%Show the corresponding heatmaps for the 61 errors and 84 head errors. PUT pictures for ENC and HEAD errors.
To validate our technique for error localization, we employ a mutation-based approach by manually introducing errors in the encoder or the head of ResNet18 by randomizing the weights of a small set of neurons. 
If our technique is valid, then by introducing errors in the encoder, the localization should result in statistically more encoder errors than head errors, and vice versa.
%\nina{It feels to me that we need to explain what exactly we expect to evaluate using mutations.} 
From ResNet18, we created two different mutated models, one with randomized weights for two neurons in each convolutional layer in the encoder, and one with randomized weights introduced only in the final classification layer, i.e., in the head. From row 2 of Tbl.~\ref{tab:enc_head_errors}, we can see that introducing mutations in the encoder resulted in significantly more encoder errors than head errors, as expected. Similarly, from row 3, mutations in the head resulted in significantly more head errors than encoder errors, as expected. 
%From row 2 of Tbl.~\ref{tab:enc_head_errors}, we can see that compared to row 1 for the original ResNet18, the number of encoder errors, identified by our localization technique, significantly increased \divya{compared to what?}\caroline{added} after introducing mutations in the encoder. Similarly, shown in row 3 of Tbl.~\ref{tab:enc_head_errors}, head errors identified by our localization technique significantly increased after mutations in the head. 
%\divya{If I understand correctly, we want to say that in row 2 , our technique identifies more encoder errors than head errors which is in alignment with the ground-truth since the mutation is only in the encoder. It is the reverse in row 3, which is also in alignment with the ground-truth. Is this correct?} \caroline{yes, I reworded these sentences a bit}
This suggests that our localization approach, although not perfect, can be useful in localizing the errors either in the encoder or the head.%}the number of encoder and head errors can indicate the location of errors in the vision model. 
% \caroline{discuss the reason for increasing head error when encoder is mutated and the other way. head is dependent on an encoder? more fine-grained localization is required?}

We attempt to determine if our localization approach can perform a more precise layer-wise localization. %A more precise localization can be conducted with two different encoder head decompositions of the same vision model. 
For example, to localize errors specifically in Residual Block 3 as shown in Fig.~\ref{fig:resnet18-decomp}, we can consider an alternative decomposition for ResNet18 by moving Residual Block 3 from the encoder to the head. %Now, the encoder contains the initial layers, Residual Blocks 0, 1, 2, and the head contains layers from Residual Block 3 on. 
In this case, mutations introduced specifically in Residual Block 3 would be encoder errors with the original decomposition, but head errors with the alternative decomposition. 
Since all Residual Blocks contain convolutional layers, to obtain an accurate $r_{map}$, we added average pooling to reduce the dimensionality of the output of Residual Block 2 before the mapping to CLIP embedding space\footnote{The resulting mapping has MSE of 1.128 and $R^2$ of 0.749, comparable with mapping obtained for the original decomposition}. %\caroline{should we discuss limitations of mapping to CLIP somewhere earlier (like background?)} 
%\susmit{Counts in Table 1 are good but they are missing the containment information. Are all 4271 reported encoder errors in Mutation in Encoder contained in reported head error in Mutation in Head? Another way to look at it would be to report false positive and false negative numbers.} \caroline{Thank you for the suggestion! Sorry I'm not sure I understand completely. Mutation in the head and encoder resulted in two different models, thus the errors are different, I am not sure if this is what you mean and I am not sure what would be the containment information in this case. For false positive/negative numbers, do you mean whether a misclassification was indeed encoder/head error? We don't really have the ground truth for this so we don't have these numbers. We can validate encoder/head error with heatmaps, encoder errors would cause the predicate to look very different. I clarified this in 4.3.3, please check. thank you. }

%\divya{[Suggestion] The last row of Tbl.~\ref{tab:enc_head_errors} shows the number of errors identified as encoder and head errors for the original and alternate decompositions respectively. Counter-intuitively, we find that irrespective of the buggy layer being present as part of the encoder or the head, the number of errors identified as head errors are more than encoder errors. However, the number of encoder errors with the original decomposition is more than the alternate decomposition, indicating a shift in the location of the bug. This highlights the potential of our algorithm with different encoder-head decompositions to precisely locate the buggy layer. However, we leave more detailed evaluation of this for future work.}

The bottom row of Tbl.~\ref{tab:enc_head_errors} presents the number of encoder and head errors with the original and alternate decomposition. Surprisingly, we observe that regardless of the location of the mutation, regardless of whether the mutation is in the encoder or the head, the number of head errors exceeds encoder errors. At the same time, the original decomposition yields more encoder errors compared to the alternate decomposition, indicating a shift in the location of the mutation. This underscores the potential of employing different encoder-head decompositions for precise layer-wise error localization. %Nonetheless, we leave a more comprehensive evaluation addressing the increase in head errors as future work.
%\nina{Do we need last sentence? This is the second time we say that we leave smth to as  future work in evaluation}\ravi{I think we should remove the sentence}
%From the last row of Tbl.~\ref{tab:enc_head_errors}, we can see that around 800 encoder errors become head errors when we switch from the original decomposition to the alternative decomposition, indicating errors specifically located in Residual Block 3. 
%However, counter-intuitively, regardless of the location of the mutation, the number of head errors significantly increased. 
%We noticed that mutation in one location can also increase errors in another location, e.g., the increase in head errors after mutating the encoder. More fine-grained and detailed analysis is required for more precise localization and repair. 


%\caroline{Reason for the increase in head errors?}
%Similar to before, shown on the right side of Tbl.~\ref{tab:enc_head_errors}, the difference in decomposition does affect the localization of errors in the encoder and head, as mutations in the encoder and head led to a significant increase in the number of encoder and head errors. 
%in order to obtain an accurate mapping before mapping the embedding to CLIP space. 

%Intuitively, given a misclassified input image $x$, we consider the error to be either 1) in the image encoder $f_{enc}$ if the embedding of this image does not correspond to the actual features in the image, e.g., wheels in the images incorrectly mapped to the embedding space of beaks, or 2) in the classification head $f_{head}$ if the image is encoded to the correct space, but the head outputs the incorrect label, e.g., incorrectly classifying an embedding of beaks as a truck which does not have beaks. 

%Given input $x$ with ground truth $c_0 \in C$ such that $f(x)\neq c_0$ (vision model misclassifies) and $g(x) = c_0$ (VLM does not misclassify), 
%let $e1 = r_{map}(f_{enc}(x))$ refer to the embedding of $x$ mapped to the VLM embedding space, $e2 = g^{img}_{enc}(x)$ refer to the embedding of $x$ directly produced by the VLM. The error is in $f_{enc}$ if $g_{head}(e1) \neq g_{head}(e2)$, and in $f_{head}$ otherwise. 

%We want to determine if the bug is located in the ENC or HEAD? Can be followed with repair or fine-tuning of the either encoder or header or a specific layer.
%{\it FL results for (i) mis-classified in-dist inputs, (ii) adv , (iii) natural perturbations, (iv) poison  \blue{added, see Tbl.~\ref{tab:enc_head_errors}}\it}
%Explain ENC or Head errors.
%The respective GT heatmaps for ENC and HEAD errors serve as validation for the FL results.

%Experiment:
%\begin{itemize}
%    \item decomposition used
%    \item Mutation-based approach: introducing errors in different parts of the model (head, enc or a specific part using two decompositions)
%    \item check the number of errors in the encoder or head
%    \item use heatmaps to validate: part with errors would show more random heatmaps
%\end{itemize}

%Results we have: (detecting error in enc or head) resnet18, resnet50, vit (soon); (layerwise with two decomposition) resnet18 



\begin{table}[t]
    \centering
    \caption{Number of encoder and head errors found through error localization for all images in the test set. }
    \label{tab:enc_head_errors}
    \scalebox{0.82}{
    \begin{tabular}{|c|>{\columncolor{tuftsblue!15}}c|>{\columncolor{turquoisegreen!20}}c|}
        \hline
        %\multirow{ 2}{*}{Mutation location}
        %& \multicolumn{2}{|c|}{Original decomposition} & \multicolumn{2}{|c}{Alternative decomposition} \\
        %\cline{2-5}
        Mutation location& \# encoder error & \# head error \\%& \# enc error & \# head error\\
         \hline
         No mutation (original ResNet18) & 61 & 84 \\%& 80 & 65 \\
         \hline
         Mutation in Encoder & 4271 & 405 \\%& 3361 & 1305\\
         \hline
         Mutation in  Head & 101 & 4571 \\%& 525 & 4147\\
         \hline
         Mutation in Residual Block 3 & \shortstack{1183 (orig decomp)\\ 438 (alt decomp)} & \shortstack{3064 (orig decomp)\\ 3809 (alt decomp)}  \\%& 438 & 3809 \\
         \hline
    \end{tabular}}
    
\end{table}

%{\it Differential GT Heatmap for in-dist ENC errors \blue{added, see Fig.~\ref{fig:fl}, in both cases, the heatmap looks like correctly classified cats but relevant concepts are not detected}\it}
\begin{figure*}[t]
    \centering
    \begin{subfigure}[t]{0.23\linewidth}
        \centering
        \includegraphics[width=\linewidth]{heatmaps/decomp/resnet18_1_class_truck_enc_error_gt.png}
        \vspace{-0.25in}
        \caption{With mutated encoder. }
        \label{sfig:fl_enc}
    \end{subfigure}
    \hspace{0.1in}
    \begin{subfigure}[t]{0.23\linewidth}
        \centering
        \includegraphics[width=\linewidth]{heatmaps/decomp/resnet18_2_class_truck_enc_error_gt.png}
        \vspace{-0.25in}
        \caption{With mutated head.}
        \label{sfig:fl_head}
    \end{subfigure}
    \hspace{0.1in}
    \begin{subfigure}[t]{0.23\linewidth}
        \centering
        \includegraphics[width=\linewidth]{heatmaps/decomp/resnet18_3_class_truck_head_error_gt.png}
        \vspace{-0.25in}
        \caption{With mutated Residual Block 3 using the original decomposition (mutations in the encoder).}
        \label{sfig:fl_rb}
    \end{subfigure}
    \hspace{0.1in}
    \begin{subfigure}[t]{0.23\linewidth}
        \centering
        \includegraphics[width=\linewidth]{heatmaps/decomp/resnet18_1_3_class_truck_enc_error_gt.png}
        \vspace{-0.25in}
        \caption{With mutated Residual Block 3 using the alternative decomposition (mutations in the head).}
        \label{sfig:fl_rb2}
    \end{subfigure}
    \vspace{-0.1in}
    \caption{Ground-truth summary heatmaps for images with ground truth \textit{truck} for various mutated ResNet18 models. The red outline indicates relevant strength predicates for class \textit{truck}. }
    \label{fig:fl}
\end{figure*} 


%\begin{comment}
 
\begin{figure*}
    \centering
    \begin{subfigure}[0.3\linewidth]
        \centering
        \includegraphics[width=\linewidth]{}
        \caption{}
        \label{}
    \end{subfigure}
    \label{fig:enter-label}
\end{figure*}   
%\end{comment}

\subsubsection{Validating Localization and Analyzing Errors with Heatmaps} 
%\caroline{summary of this paragraph: heatmaps can be used to verify encoder vs head errors. for gt truck images, if relevant strength predicates are sat, encoder is correct, error is likely in head, else, error is likely in the encoder }

With semantic heatmaps, we can visualize and validate localization results and understand the reasons for failure. Heatmaps show the satisfaction of the strength predicates by the output of the encoder, i.e., the image embedding. %Therefore, with encoder errors, the satisfaction of strength predicates would be different than expected in ground truth, e.g., an inaccurate embedding of truck images would not satisfy relevant strength predicates for trucks. If the errors are only in the head, the satisfaction of strength predicates would be similar to ground truth. 
For \textit{truck} images misclassified by the original ResNet18, from Fig.~\ref{sfig:truck_enc}, we can observe that, compared to correctly classified images in Fig.~\ref{sfig:correct_truck}, a few relevant strength predicates have lower satisfaction probability, e.g., $text>patterned$, %$wheels>tail$, $wheels>patterned$,
as well as the ones involving relevant concepts $wheels$ and $tail$;  
%\divya{looks like all relevant strength predicates with wheel as con1, or tail as con2 have lower satisfaction probabilities} \caroline{added in the text} , 
and several non-relevant strength predicates have higher satisfaction, e.g., $ears>mane$, indicating encoder errors. On the other hand, Fig.~\ref{sfig:truck_head} highly resembles Fig.~\ref{sfig:correct_truck}, suggesting the images are correctly encoded and thus the errors are in the head.
%\divya{ maybe we should move the above discussion about the heatmaps to 4.3.3?} \caroline{moved}

Next, to validate localization and further analyze failures of the mutated ResNet18 models, we constructed ground-truth summary heatmaps for images with ground truth truck (Fig.~\ref{sfig:fl_enc}-\ref{sfig:fl_rb2}). We can see in Fig.~\ref{sfig:fl_enc}, with the mutated encoder, many relevant strength predicates for trucks have low satisfaction probability, indicating errors in the image embedding as expected. Specifically, predicates involving \textit{wheels} and \textit{text} have the lowest satisfaction probability, suggesting the encoder is not identifying these specific concepts from the input images. However, with the mutated head, as shown in Fig.~\ref{sfig:fl_head}, relevant strength predicates are still satisfied with high probability, indicating errors are more likely to be in the classification head rather than the encoder, as predicted. For mutated Residual Block 3, with the original decomposition, it is part of the encoder, thus Fig.~\ref{sfig:fl_rb} shows decreased satisfaction probability in a few relevant strength predicates, e.g., $wheels>tail$ and $text>hairy$; with the alternative decomposition, it is part of the head, thus Fig.~\ref{sfig:fl_rb2} shows most relevant predicates are still satisfied with high probability. 

%\caroline{these are future directions?}
%Can help focus testing and repair; generate test inputs that satisfy the violated predicates, repair the encoder to satisfy the violated predicates for the failing inputs. 


\begin{figure*}[t]
    \centering
    \begin{subfigure}[t]{0.23\linewidth}
        \centering
        \includegraphics[width=\linewidth]{heatmaps/decomp/pgd_truck.jpg}
        \vspace{-0.25in}
        \caption{Ground-truth heatmap for all perturbed images (PGD with $l_{\infty}$). }
        \label{sfig:rf_pgd}
    \end{subfigure}
    \hspace{0.05in}
    \begin{subfigure}[t]{0.23\linewidth}
        \centering
        \includegraphics[width=\linewidth]{heatmaps/decomp/pgd_diff_truck.jpg}
        \vspace{-0.25in}
        \caption{Differential heatmap displaying the absolute difference between Fig.~\ref{sfig:correct_truck} and Fig.~\ref{sfig:rf_pgd}.}
        \label{sfig:rf_diff}
    \end{subfigure}
    \hspace{0.05in}
    \begin{subfigure}[t]{0.23\linewidth}
        \centering
        \includegraphics[width=\linewidth]{heatmaps/decomp/pgdl2_truck.jpg}
        \vspace{-0.25in}
        \caption{Ground-truth heatmap for all perturbed images (PGD with $l_2$). }
        \label{sfig:rf_pgd2}
    \end{subfigure}
    \hspace{0.05in}
    \begin{subfigure}[t]{0.23\linewidth}
        \centering
        \includegraphics[width=\linewidth]{heatmaps/decomp/pgdl2_diff_truck.jpg}
        \vspace{-0.25in}
        \caption{Differential heatmap displaying the absolute difference between Fig.~\ref{sfig:correct_truck} and Fig.~\ref{sfig:rf_pgd2}.}
        \label{sfig:rf_diff2}
    \end{subfigure}
    \vspace{-0.1in}
    \caption{Heatmaps for identifying robust and non-robust features against Projected Gradient Descent (PGD) attack (both $l_{\infty}$ and $l_2$). All heatmaps consider images with ground truth \textit{truck}. The black outline shows robust strength predicates where the absolute difference in satisfaction probability $\leq0.05$. The red outline indicates relevant strength predicates for class \textit{truck}.}
    \label{fig:rf}
\end{figure*}   

\subsection{Application 3: Identification of Robust and Non-robust Strength Predicates}
\label{subsec:robust_feat}
%\caroline{summary of this paragraph: we can identify features (that are the satisfaction of strength predicates) robust in the presence of adv perturbations. we show heatmaps for a perturbation resnet18 is robust to (pgd l2) and one it is not (pgd $l_{\infty}$)}

%Vision models can be vulnerable to adversarial perturbations, i.e., small perturbations in the inputs can cause misclassification~\cite{Szegedy2014IntriguingPO}, thus robustness analysis is necessary for risk assessment of vision models. Concept-based analysis allows us to extend analysis beyond accuracy and identify strength predicates that can and cannot be robustly satisfied by the vision models in the presence of adversarial perturbations, which is important for understanding the predictability and adaptability of the vision models. A strength predicate is robust against a perturbation if the satisfaction probability (that is $>0$) remains the same before and after applying the perturbation, and non-robust otherwise. 
%\corina{do we explain anywhere why finding robust/non robust features is important? perhaps in intro?}

%\divya{In the section below, shouldn't we be referring to Figures 3a for the heatmaps for non-perturbed truck images? Fig 3b is the subset of truck images which are also correctly classified.}\caroline{yes, corrected}

With ResNet18, Fig.~\ref{fig:all_truck}  shows the ground-truth summary heatmap obtained with all original \textit{truck} images without any perturbations, and Fig.~\ref{sfig:rf_pgd} shows the heatmap obtained with all \textit{truck} images perturbed with Projected Gradient Descent (PGD) (perturbation radius $ \epsilon=\frac{8}{255}$)~\cite{MadryMSTV18}. ResNet18 has a $0\%$ accuracy on all perturbed images, i.e., not robust against the $l_{\infty}$ PGD attack. This is also evident in Fig.~\ref{fig:all_truck} and Fig.~\ref{sfig:rf_pgd}---the satisfaction of most strength predicates is affected by the perturbation. By visualizing the absolute difference between these two heatmaps (see Fig.~\ref{sfig:rf_diff}, lighter green indicates a smaller difference), we can identify a small set of strength predicates that remained constant, i.e., with absolute difference $\leq 0.05$, that are robust predicates, e.g., %$ears>beak
$rectangular>horns,~long>ears$, and the rest are non-robust predicates, e.g., $wheels> tail,~%rectangular>tail$
metallic > long-snout$. Notice that the majority of all relevant strength predicates for \textit{trucks} are not robust, suggesting ResNet18 is not robust against $l_{\infty}$ PGD.
%\divya{mention some more robust and non-robust features}. 
Additionally, considering the $l_{2}$ PGD attack ($\epsilon=\frac{8}{255}$), ResNet18 is robust---it has a $96.3\%$ accuracy on all perturbed images. In addition to high accuracy, we can validate using the heatmap obtained for all \textit{truck} images perturbed with $l_{2}$ PGD attack(Fig.~\ref{sfig:rf_pgd2}) as well as the differential heatmap between Fig.~\ref{fig:all_truck} and Fig.~\ref{sfig:rf_pgd2}. We see that ResNet18 can robustly satisfy all of the strength predicates. 
%In this case, all the non-robust predicates have satisfaction probability $0$ before and after the perturbation. \ravi{i dont understand why these are being called non-robust? Isnt a predicate non-robust only if there is a big change in satisfaction probability after perturbation?} 
%\divya{point out non-robust features if any. Some irrelevant predicates have a large difference example floppy-ears - mane, rectangular - wheels. Mention that these do not impact model output for truck.} 
By analyzing model robustness through concepts, we assign meaning to statistical results, allowing us to better understand the effects of the adversarial perturbations, and thus allowing developers to design more meaningful detectors and attacks.

Additionally, this experiment highlights that most adversarial examples get misclassified due to encoder errors. 
While the encoder of ResNet18 is nearly accurate for in-distribution inputs, adversarial perturbations can lead to incorrect encoding as suggested by the non-robust features. Such insights can facilitate re-training or repair efforts by directing attention to the encoder and the specific non-robust strength predicates.


%Tail is a concept, $tail > metallic$ is a feature. 
%Identify invariant properties. 
%Can help re-training with focus on the non-robust features. 

%Experiment:
%\begin{itemize}
%    \item plot heatmaps w.r.t. ground truth before and after perturbations, 
%    \item highlight features ``preserved'' (diff $\leq threshold$) 
%\end{itemize}

%\blue{Results are shown in Fig.~\ref{fig:rf}.}

%Results we have: (adv) pgd, fab, fgsm, pgdl2, mix, (natural) brightness%, (poison) gradient matching, \red{can run more if needed}

\begin{figure*}[t]
    \centering
    \begin{tabular}{ccc}
    \begin{subfigure}[t]{0.3\linewidth}
        \centering
        \includegraphics[width=\linewidth]{heatmaps/decomp/pgd_truck_outout.jpg}
    \vspace{-0.25in}
    \caption{Output-label summary heatmap for perturbed images classified as \textit{truck}.}
    \label{sfig:detect_pgd}
    \end{subfigure} &
    \begin{subfigure}[t]{0.3\linewidth}
        \centering
        \includegraphics[width=\linewidth]{heatmaps/decomp/correct_pgd_truck_bin.jpg}
    \vspace{-0.25in}
    \caption{Binarized heatmap of correctly classified clean images of \textit{trucks} (binarized Fig.~\ref{sfig:correct_truck}). }
    \label{sfig:detect_c}
    \end{subfigure}&
    \begin{subfigure}[t]{0.3\linewidth}
        \centering
        \includegraphics[width=\linewidth]{heatmaps/decomp/pgd_truck_bin.jpg}
        \vspace{-0.25in}
        \caption{Binarized heatmap of perturbed images classified as \textit{truck} (binarized Fig.~\ref{sfig:detect_pgd}). }
        \label{sfig:detect_pgd_b}
    \end{subfigure}\\
    \end{tabular}
    \vspace{-0.1in}
    \caption{Heatmaps used for runtime detection of adversarial inputs with ResNet18. Adversarial inputs generated with $l_{\infty}$ PGD attack, $\epsilon=\frac{8}{255}$. Fig.~\ref{sfig:detect_c} and Fig.~\ref{sfig:detect_pgd_b} binarized with threshold $0.6$. Red outlines indicate relevant strength predicates for class \textit{truck}. }
    \label{fig:fl}
    %\vspace{-0.1in}
\end{figure*} 

\begin{table*}[t]
    \centering
    \caption{Accuracy for detecting adversarial inputs vs clean inputs with heatmaps for all images in the test set. For each class $c$, we have about 500 clean images with ground truth $c$ and 500 perturbed images that are labeled by ResNet18 as $c$. Each cell contains ($a_p$, $a_n$) where $a_p$ is the percentage of perturbed images correctly detected as adversarial inputs ($IoU_p > IoU_n$), and $a_n$ percentage of clean images correctly detected ($IoU_p \leq IoU_n$). $\epsilon$ is $\frac{8}{255}$ for all experiments.}
    \label{tab:adv_acc}
    \vspace{0.05in}
    \begin{tabular}{cccccc}
    \toprule
        & \shortstack{PGD $l_{\infty}$} & \shortstack{FAB $l_{\infty}$} & \shortstack{FGSM $l_{\infty}$} & \shortstack{PGD $l_{2}$} & \shortstack{Mixture}\\
         \midrule
         \textit{truck} & (0.943 , 0.497) & (0.961 , 0.647) & (0.930 , 0.887) & (0.779 , 0.256) & (0.793 , 0.529)\\
        \textit{car} & (0.977 , 0.522) & (0.990 , 0.577) & (0.932 , 0.730) & (0.893 , 0.112) & (0.936 , 0.653)\\
        \textit{plane} & (0.913 , 0.627) & (0.952 , 0.694) & (0.950 , 0.805) & (0.890 , 0.127) & (0.944 , 0.725)\\
        \textit{ship} & (0.886 , 0.732) & (0.901 , 0.757) & (0.941 , 0.929) & (0.718 , 0.301) & (0.901 , 0.783)\\
        \textit{cat} & (0.479 , 0.937) & (0.938 , 0.802) & (0.915 , 0.706) & (0.866 , 0.146) & (0.535 , 0.800)\\
        \textit{dog} & (0.787 , 0.593) & (0.960 , 0.618) & (0.950 , 0.600) & (0.880 , 0.137) & (0.813 , 0.526)\\
        \textit{equine} & (0.552 , 0.871) & (0.901 , 0.819) & (0.903 , 0.866) & (0.872 , 0.161) & (0.771 , 0.707)\\
        \textit{deer} & (0.921 , 0.614) & (0.939 , 0.720) & (0.947 , 0.856) & (0.867 , 0.152) & (0.939 , 0.675)\\
        \textit{frog} & (0.865 , 0.658) & (0.910 , 0.634) & (0.940 , 0.716) & (0.904 , 0.117) & (0.856 , 0.627)\\
        \textit{bird} & (0.795 , 0.558) & (0.964 , 0.794) & (0.962 , 0.640) & (0.972 , 0.034) & (0.816 , 0.613)\\
        \hline
        Total & (0.810 , 0.663) & (0.941 , 0.711) & (0.937 , 0.764) & (0.864 , 0.154) & (0.830 , 0.681)\\
         \bottomrule
         \multicolumn{5}{l}{*All numbers are rounded.}
    \end{tabular}
    \vspace{-0.1in}
\end{table*}

\subsection{Application 4: Runtime Detection of Adversarial Inputs}
\label{subsec:adv_detect}
%\caroline{Summary of this paragraph: run time detection can be done by comparing each single-input heatmap with summary heatmaps of 1) correctly classified original images of a class; 2) perturbed images misclassified to this class. The comparison can be done by simply binarizing summary heatmaps with a threshold, and using IoU to determine whether each single-input heatmap is more similar to heatmap 1) or heatmap 2). Using CLIP directly can give more accurate results, but CLIP is too expensive for runtime detection. }

%\corina{do we explain anywhere what adversarial inputs are and why it is important to detect them??}

So far, we have primarily relied on the ground-truth summary heatmaps for interpreting model behaviour. When ground truth information is unavailable, e.g., during runtime, we can utilize output-label summary heatmaps for analysis, for instance, enabling runtime detection of adversarial inputs. As we observed before, adversarial perturbations lead to encoder errors. Therefore, with output-label summary heatmaps of a particular class, the relevant strength predicates would appear satisfied. 
%Intuitively, perturbations can affect the encoding of concepts in the inputs, therefore, heatmaps for non-perturbed images of one class would be different from heatmaps for perturbed images classified to the same class.
%Adv detectionL since adv perturbations lead to encoder errors, when look at output based heatmaps for a label, the relevant predicate gets satisfied by both miusclassifie and correctly classified; but the not-relevant are different. Since they were mapped from other classes, giving random satisfaction rate. We zoom in on this, thus we use single-output and then …. Reason this relevant seems same with perturbat, previously, adv lead to lots of encoder errors.
For example, consider PGD $l_{\infty}$  attack ($\epsilon=\frac{8}{255}$); Fig.~\ref{sfig:detect_pgd} shows the summary heatmap for all perturbed images misclassified to \textit{truck} by ResNet18. Most relevant strength predicates for \textit{trucks} are satisfied since these images are classified as \textit{trucks}. However, since these images are incorrectly mapped to \textit{trucks} from other classes, the strength predicates not relevant to \textit{truck} but that are relevant for other classes, show a more different and random satisfaction rate. Zooming in on this for adversarial detection, for each input, we identify such differences in its single-input heatmap.%\divya{single-input heatmap} 
%Compared to Fig.~\ref{sfig:rf_c}, the satisfaction of most strength predicates is affected by the perturbation and differs from that of non-perturbed images. 
%We demonstrate that adversarial inputs can be detected during runtime by identifying such differences.


First, for each output class, we construct a ground-truth summary heatmap with all clean images (i.e., a clean heatmap as in Fig.~\ref{sfig:correct_truck} for \textit{truck}) 
%\ravi{Do we conside ground-truth heatmaps or output heatmaps for clean images? Seems like we should consider output heatmaps} 
and a output summary heatmap with all adversarial inputs generated during offline analysis (i.e., a perturbed heatmap as in Fig.~\ref{sfig:detect_pgd} for \textit{truck}). Then, for each input encountered during runtime with output class $c$, this input is considered adversarial if its single-input heatmap is more similar to the perturbed heatmap than the clean heatmap of class $c$, and clean otherwise. To determine the similarity between a single-input heatmap and the above summary heatmaps,
%\susmit{is summary over all of training data - different inputs have different heatmaps}\caroline{addressed}, 
we first binarize the summary heatmap with a threshold $t$ %\susmit{some insight into selection of t would be useful}\caroline{added after this sentence, please check} 
to highlight strength predicates with high satisfaction probabilities, i.e., $1$ if satisfaction probability $\geq t$, and $0$ otherwise. 
The value of $t$ should be sufficiently high to capture the primary differences between clean and perturbed heatmaps while avoiding the inclusion of small values that are predicates satisfied by only a small set of images. In our experiment, we set 
$t=0.6$, which resulted in the highest detection accuracy.
The binarized clean heatmap (binarized Fig.~\ref{sfig:correct_truck}) is shown in Fig.~\ref{sfig:detect_c}; and the binarized perturbed heatmap (binarized Fig.~\ref{sfig:detect_pgd}) is shown in Fig.~\ref{sfig:detect_pgd_b}, with $t=0.6$. Then we compute Intersection over Union (IoU) as the similarity metric, between each single-input heatmap and the binarized summary heatmaps; we use $IoU_p$ for similarity with the the binarized perturbed heatmap, and $IoU_n$ for similarity with the binarized clean heatmap. An input with $IoU_p > IoU_n$ suggests it is adversarial, and clean otherwise.


To demonstrate runtime detection of adversarial inputs, 
%we considered common adversarial perturbations 
we constructed sets of perturbed inputs (all with $\epsilon=\frac{8}{255}$) using common adversarial attacks such as 
PGD (both $l_{\infty}$ and $l_2$)~\cite{MadryMSTV18}, FGSM ($l_{\infty}$)~\cite{Szegedy2014IntriguingPO}, FAB ($l_{\infty}$)~\cite{croce2020minimally}, and a random mixture of all the above. In Tbl.~\ref{tab:adv_acc}, we show the accuracy of identifying perturbed from clean images per class. Overall, we were able to achieve high accuracy for most classes and most perturbations with a simple similarity metric. This suggests our heatmaps have the potential for more precise runtime detection. For PGD $l_2$ with lower accuracy in Tbl.~\ref{tab:adv_acc}, as we showed in Sec.~\ref{subsec:robust_feat}, ResNet18 is robust against PGD $l_2$ with high robust accuracy, thus the perturbed and clean heatmaps are too similar for differentiating adversarial inputs. Additionally, we noticed that adversarial attacks affect different classes differently---classes with lower accuracy have more similar perturbed and clean heatmaps,
%\ravi{this contradicts the previous statement that suggests that if the model performance is similar for clean and adv inputs, i.e., model is robust, then heatmaps are similar},
suggesting the model is more robust for some classes of inputs than others. 
%Overall these results suggest that our adversarial detector works better when the model is less robust since the clean and adversarial heatmaps are very similar in these cases.

%we only used images clip correctly classified. Attack works differently for different classes: classes with low accuracy have similar heatmaps between original and perturbed data (model is robust).
Note that VLMs such as CLIP can themselves be deployed as runtime detectors to catch inputs misclassified by the vision model. CLIP has robust accuracy $0.982$ against PGD $l_{\infty}$, $0.984$ against FAB, $0.973$ against FGSM, and $0.984$ against PGD $l_{2}$, all of which are higher than detection accuracy with semantic heatmaps. However, foundation models such as CLIP are too computationally heavy to be deployed during runtime, while our heatmaps can be precomputed, only the single-layer linear aligner $r_{map}$ is required during runtime, which is more desirable for analysis during runtime. 



%However, our concept-based detection technique is more desirable due to the following reasons; (i) Foundation models such as CLIP are heavy-weight to deploy at runtime, (ii) The zero-shot classification of CLIP is not 100\% so the runtime ``oracle" may be wrong. On the other hand, the concept-based heatmaps are built only using instances on which CLIP is 100\% accurate, further they employ finer-grained information in terms of concepts. Hence this technique has the potential to have more precise detection


%We describe offline analysis of r such inputs.
%\blue{also show results for directly using CLIP}
%CLIP acc:
%\begin{itemize}
%    \item pgd: 0.9820279984865683
%    \item fab: 0.9841089670828603
%    \item fgsm: 0.9729474082482028
%    \item pgdl2: 0.9844873250094589
%    \item mix: 0.9752175558077941
    %\item brightness: 0.14812712826333713
%\end{itemize}



%\subsubsection{Adv data}

%Experiment \blue{see Fig.~\ref{fig:adv} and Tbl.~\ref{tab:adv_acc} (using images that CLIP correctly classified)}:
%\begin{itemize}
%    \item plot heatmaps w.r.t. model output before and after perturbations
%    \item detection by comparing IoU with original heatmap and perturbed heatmaps
%    \item best results achieved together with robust features
%\end{itemize}

%Additional observations: 
%\begin{itemize}
    %\item CLIP is not robust to natural perturbations like brightness: images misclassified by the model are also misclassified by CLIP
    %\item Attack works differently for different classes: classes with low accuracy have similar heatmaps between original and perturbed data (model is robust). 
    %\item CLIP is not robust to natural perturbations
    %\item natural perturbations can be detected (heatmaps are quite different), but detecting misclassification like adv is harder
%\end{itemize}

%Results we have: (adv) pgd, fab, fgsm, pgdl2, mix, (natural) brightness





%\subsubsection{Poisoned data}
%Previously, people showed that for poisoned data, the model uses different features, and different groups of neurons are activated than the original data. We can assign meaning to these features, verify the assumption of previous work and give explanations of model behaviour. 


%\subsection{Future Directions}
%\caroline{summary of future work: repair, data selection for retraining, adv detection, etc. }
%\caroline{summary of discussion: in error localization, introducing errors in head also increased encoder errors, further analysis is required; the clip version we used is not robust to natural perturbations, e.g., brightness}


%Our results can assist testing and repair of the vision models, and enable more localized repair. 

%in localization, other error increases 

%Bugs localization and visualization with heatmaps can help with testing and repair of the vision models, including test generation focusing on violated predicates, and localized repair.




%\begin{comment}
    
\begin{figure*}[t]
    \centering
    \begin{subfigure}{0.3\linewidth}
        \centering
        \includegraphics[width=\linewidth]{heatmaps/detection/correct_truck.jpg}
        \caption{Truck images correctly classified.}
        \label{sfig:adv_c}
    \end{subfigure}
    \hspace{0.1in}
    \begin{subfigure}{0.3\linewidth}
        \centering
        \includegraphics[width=\linewidth]{heatmaps/detection/pgd_truck.jpg}
        \caption{PGD Linf.}
        \label{sfig:adv_pgd}
    \end{subfigure}
    \hspace{0.1in}
    \begin{subfigure}{0.3\linewidth}
        \centering
        \includegraphics[width=\linewidth]{heatmaps/detection/fab_truck.jpg}
        \caption{Fab Linf.}
        \label{sfig:adv_fab}
    \end{subfigure}
    \hspace{0.1in}
    \begin{subfigure}{0.3\linewidth}
        \centering
        \includegraphics[width=\linewidth]{heatmaps/detection/fgsm_truck.jpg}
        \caption{FGSM Linf.}
        \label{sfig:adv_fgsm}
    \end{subfigure}
    \hspace{0.1in}
    \begin{subfigure}{0.3\linewidth}
        \centering
        \includegraphics[width=\linewidth]{heatmaps/detection/pgdl2_truck.jpg}
        \caption{PGD L2.}
        \label{sfig:adv_pgdl2}
    \end{subfigure}
    \hspace{0.1in}
    \begin{subfigure}{0.3\linewidth}
        \centering
        \includegraphics[width=\linewidth]{heatmaps/detection/mix_truck.jpg}
        \caption{Mixture of perturbations in Fig.~\ref{sfig:adv_pgd} to Fig.~\ref{sfig:adv_pgdl2}.}
        \label{sfig:adv_mix}
    \end{subfigure}
    \caption{Heatmaps of images with different types of adversarial attacks misclassified as truck. }
    \label{fig:adv}
\end{figure*}       

%\end{comment}

==> sections/applications_old.tex <==
\section{Analysis Results}

\subsection{Application 1: Explaining Behavior}
\label{subsec:explain_beh}
%\caroline{summary of this paragraph: heatmaps help visualize whether outputs are produced for the right reasons.}
%\corina{do we explain anywhere why explaining correct behaviour is useful? perhaps in intro?}
Given inputs that are correctly classified by the vision model, i.e., model output matches the ground truth, 
%Given a set of inputs on which the model produces outputs matching the ideal label, 
we aim to understand if the model produces these outputs for the \textit{right reasons}, which helps build trust in the behavior of the model beyond testing. Using our semantic heatmaps, we can visualize concepts utilized by the model for producing these outputs. 

We use images and concepts related to class \textit{truck} to illustrate our ideas.
Fig.~\ref{sfig:correct_truck} 
%To visualize concepts in inputs that led to the output \textit{truck} by ResNet18, in Fig.~\ref{sfig:correct_truck}, 
%we show the summary heatmap constructed with all \textit{truck} images from the RIVAL10 test set correctly classified by ResNet18.
%we show the
depicts the ground-truth summary heatmap computed with all \textit{truck} images from the RIVAL10 test set that are correctly classified by ResNet18. %\ravi{made minor edit, please check}
%\ravi{This kind of summary heatmap is not convered under any of the three different kinds we disucssed in the previous section. Should we merge ground truth based and output label based?}
From the heatmap, we see that ResNet18 can satisfy most relevant predicates, i.e., the ones involving concepts relevant to \textit{trucks} (highlighted with red outlines) with high probability, 
%satisfaction probability of relevant concepts (highlighted with red outlines) 
except for the predicate $metallic>tail$, and predicates involving concept \textit{text}, e.g., $text>tail$ and $text>horns$. 
%This suggests that ResNet18 can indeed identify objects that are \textit{long, rectangular, tall,} and \textit{metallic} with \textit{wheels} as \textit{trucks}; but struggles to effectively identify text in images, and distinguish \textit{metallic} and \textit{tails}. \ravi{From Fig 3b, we can only draw conclusion about model behavior on trucks, so this sentence seems too strong. }
This suggests that when ResNet18 correctly classifies images as \textit{trucks}, it indeed does so for the \emph{right reasons}---it is able to recognize the strong presence of concepts such as \textit{long, rectangular, tall, metallic} with \textit{wheels} in these images. However the model struggles to effectively identify text in images, and distinguish \textit{metallic} and \textit{tails}.
Such information can facilitate performance improvements of the vision models, e.g., guiding data selection for retraining. Additionally, notice that some non-relevant predicates also have high satisfaction probabilities, e.g., $tail>beak$. This could be the result of other concepts in the images, the dependency between relevant and non-relevant concepts, or how the CLIP model is trained. Further analysis is required to determine the cause, we leave this as future work.

Fig.~\ref{fig:all_truck} shows the ground-truth summary heatmap of all images with ground-truth \textit{truck}. It is visually similar to the summary heatmap of all images correctly classified as \textit{truck} ((Fig.~\ref{sfig:correct_truck})) with most relevant strength predicates for \textit{trucks} satisfied with a high probability.  
%This suggests that ResNet18 is able to correctly encode relevant concepts in its representation space for the majority of in-distribution inputs, and this is expected due to the high accuracy of ResNet18 on these images.
%\ravi{Not very clear. Fig 3a shows us that for images with ground truth truck, model is able to correctly identify the relevant strength predicates, indicating that it is able to correctly encode relevant concepts in its representation space for the majority of in-distribution truck inputs. Given Fig 3b is very similar to Fig 3a, it further shows that when the model predicts truck correctly, it does so for the right reasons. The analysis in previous para also shows this.} 
This suggests that ResNet18 is able to correctly extract the relevant concepts  for the majority of \textit{truck} inputs, and this is expected due to the high accuracy of ResNet18 on these images.
However, in the following sections, as we delve deeper into the representation space for subsets of inputs that are incorrectly classified, we discover that the encoder incorrectly encodes a subset of inputs which leads to misclassification. 
%\susmit{A bit confusing sentence - was the incorrect encoding only for incorrectly classified inputs? If so, remove ``correctly and".}\caroline{addressed, removed ``correctly and"}

%\caroline{future directions? interpretation, data selection, finetuning?}


%{\it Heatmap for correctly classified inputs for Rival10. \blue{added, see Fig.~\ref{fig:correct_truck}}\it} 

\begin{figure*}[t]
    \centering
    \begin{subfigure}{0.23\linewidth}
        \centering
        \includegraphics[width=\linewidth]{heatmaps/resnet/all_GT_truck.jpg}
    %\vspace{-0.25in}
    \caption{With all images with ground truth \textit{truck}.}
    \label{fig:all_truck}
    \end{subfigure}
    \hspace{0.05in}
    \begin{subfigure}{0.23\linewidth}
        \centering
        \includegraphics[width=\linewidth]{heatmaps/resnet/all_correct_truck.jpg}
        \vspace{-0.25in}
        \caption{With images correctly classified as \textit{truck}. }
        \label{sfig:correct_truck}
    \end{subfigure}
    \hspace{0.05in}
    \begin{subfigure}{0.23\linewidth}
        \centering
        \includegraphics[width=\linewidth]{heatmaps/resnet/all_GT_enc_error_truck.jpg}
        \vspace{-0.25in}
        \caption{With misclassified \textit{truck} images due to encoder error.}
        \label{sfig:truck_enc}
    \end{subfigure}
    \hspace{0.05in}
    \begin{subfigure}{0.23\linewidth}
        \centering
        \includegraphics[width=\linewidth]{heatmaps/resnet/all_GT_head_error_truck.jpg}
        \vspace{-0.25in}
        \caption{With misclassified \textit{truck} images due to head error.}
        \label{sfig:truck_head}
    \end{subfigure}
    \vspace{-0.1in}
    \caption{Ground-truth summary heatmaps for \textit{truck} images. The red outline indicates relevant predicates for class \textit{truck}. }
    \label{fig:resnet-error}
    \vspace{-0.15in}
\end{figure*} 

\subsection{Application 2: Debugging and Fault Localization}
\label{subsec:debugging}

\begin{figure*}
\centering
\includegraphics[scale=0.35]{figures/ENC_HEAD_ERR_examples.png}
%\caption{Examples of misclassified inputs for ResNet18 model, localized to bug in the encoder (Encoder Error) and bug in the head (Head Error).}
\vspace{-0.1in}
\caption{Examples of misclassified inputs of ResNet18, error localized to the encoder (Encoder Error) and the head (Head Error).}
\label{fig:enc_head_errs}
\label{fig:enc_head_errs}
\end{figure*}

For inputs that are misclassified by the vision model, i.e., the model output does not match the ground truth, 
%Given a set of inputs on which the model fails, 
we wish to investigate the cause of failures, which can further aid in activities such as targeted testing and repair.%, and re-training to improve the model performance. 

%We investigate the following types of failures; mis-classified in-distribution inputs and inputs with specific types of perturbations. (this is probably not this application)
%{\it How does CLIP perform when fed directly with perturbed inputs? \it} 

%\paragraph{Setup} 
%\begin{itemize}
%    \item Dataset: Rival10
%    \item vision models: Resnet18, Resnet50, vit\_tiny, VLM: clip
%    \item t2c mappings
%    \item perturbations: adversarial, poison, natural (brightness, noise, etc.)
%\end{itemize}

\subsubsection{Localization to Encoder and Head Errors}
%\subsubsection{Encoder and Head Errors} %\caroline{summary of this paragraph: def of encoder vs head error.}
Consider an input $x$ with ground truth $c_0 \in C$ such that $f(x)\neq c_0$, i.e., misclassified by the vision model. The decomposition of the vision model into an image encoder $f_{enc}$ and a classification head $f_{head}$ (see Sec.~\ref{sec:overview}) allows us to localize errors to a specific part of the model. The misclassification can be caused by errors in the encoder, i.e., the encoder does not correctly encode relevant concepts; or errors in the head, i.e., concepts are encoded correctly but the wrong output label is produced; or both. The location of the error can be detected through strength predicates. Intuitively, if the strength predicates relevant for the ground truth label of $x$ are not satisfied by its image embedding, then the encoder has incorrectly encoded the image; otherwise, the error is in the head. %Note that with encoder errors, errors in the head may be present at the same time. However, since updating the encoder would also affect the head, the encoder errors should be addressed first, thus we consider such a case as encoder errors. 
Note that, for an image $x$, encoder and head errors may be present at the same time. However, since updating the encoder would also require updating the head, the encoder errors should be addressed first, thus we consider such cases as exclusively encoder errors. %\ravi{reworded slightly; check}
We present an %\divya{perhaps remove lighweight since we do not show that it is lightweight?}\caroline{removed} 
approach to localize errors as encoder or head errors, and then use summary semantic heatmaps to validate the localization and analyze the errors.


%As explained in section~\ref{sec:overview}, this could be caused due to an error in the encoder (does not encode relevant features correctly), or an error in the head (does encode the features correctly, but the classification head does not apply the correct logic for classification), or in both. 
%Our insight is that if there is a problem in the encoder, then the representation space should highlight this (i.e) the embedding vector corresponding to the misclassified input would not satisfy relevant strength predicates for the GT label. If the embedding vector does satisfy the relevant strength predicates, then the problem could be isolated to the head. 
%Note that, in the former case, the problem could also be in the head but we consider them as {\it encoder \it} errors, since we know for sure that there are problems in the encoder that could be addressed first.
%We could adopt the above-mentioned technique and evaluate single-input heatmaps of every misclassified input. However, every input may satisfy a different set of relevant (and) irrelevant strength predicates, which may can complicate the analysis. We present a lightweight approach to first categorize encoder and head errors, and then use summary concept heatmaps to validate the localization.

%Intuitively, if an embedding vector does not satisfy a sufficient number of strength predicates for a label, then a zero-shot classification via $g_{head}$ would not give the correct label.
%\ravi{Not sure I understand. What is embedding vector referring to here? Is it it embedding generated $f_{enc}$ or $g_{enc}$?}
%\divya{should we define formally or explain how zero-shot classification via $g_{head}$ is done?}\caroline{I think this is in background} \corina{yes it is explained in background} \divya{Since here we present an algorithm for localization using zero-shot classification, I was thinking if we should give more details or formalize $g_{head}$.} 
 
%\divya{We could directly use concept heatmap for an input to  categorize it as encoder error vs head error. Should we give some reason why we choose to use zero-shot classification instead?} \caroline{I guess the reason would be: we kind of use the VLM as the oracle in this paper, this would give us the most precise results?} 
%
%Therefore, %\caroline{assuming VLM correct added here}consider an input $x$ with ground truth $c_0$ that the VLM correctly classifies, i.e., $g_{head}(g_{enc}^{img} (x)) = c_0$ but the model misclassifies, i.e., $f(x) \neq c_0$.  
%However, to use this approach, we need to ensure that $g_{head}$  is accurate. We validate the zero-shot classification of CLIP for all test inputs (mis-classified by ResNet18); $e1 = g^{img}_{enc}(x) ; c = g_{head}(e1); c = c_{0}$ . We found the accuracy to be very high (TBD). <- I don't think we need this, we said the acc of CLIP earlier. 
%Therefore, for every input, we can then check if $e2 = r_{map}(x) ; g_{head}(e2)$ gives the correct label, or more simply if $g_{head}(e1) = g_{head}(e2)$. Subsequently, we categorize mis-classified inputs where $g_{head}(e1) \ne g_{head}(e2)$ as {\it encoder errors \it}, and  {\it head errors \it} otherwise. 
%Our concept-based analysis assumed that vision models can be decomposed into an image encoder $f_{enc}$ and a classification head $f_{head}$. This decomposition, together with the mapping from the vision model to the VLM, allows us to localize errors to a specific part of the model, i.e., encoder or head, that needs to be repaired or fine-tuned. %We can distinguish between encoder and head errors through the mapping from the vision model to the VLM. 
%Consider an input $x$ with ground truth $c_0 \in C$ such that $f(x)\neq c_0$, i.e., misclassified by the vision model, and $g(x) = c_0$, i.e., correctly classified by the VLM. 
%Intuitively, we consider the misclassification caused by errors in the encoder $f_{enc}$ if the embedding of this image does not correspond to the actual features in the image, e.g., wheels in the image incorrectly mapped to the embedding space of beaks.


Consider an input $x$ with ground truth $c_0$ that the VLM correctly classifies, i.e., $g_{head}(g_{enc}^{img} (x)) = c_0$ but the model misclassifies, i.e., $f(x) \neq c_0$.
Let $e_1 := r_{map}(f_{enc}(x))$ refer to the embedding of $x$ produced by the vision model, and let $e_2:= g^{img}_{enc}(x)$ refer to the embedding of $x$ directly produced by the VLM. 

\vspace{0.05in}
\noindent{\textit{\textbf{Localizing Encoder Error.}}}
If $e_1$ and $e_2$ lead to different zero-shot classification outputs, i.e., $g_{head}(e_1) \neq g_{head}(e_2)$, then we can localize that the error is in $f_{enc}$, we call it \textit{encoder error}. 
%\divya{should we mention we assume $g_{head}(e2)$ is correct?}\caroline{added}. 
%\end{definition}

\vspace{0.05in}
%\begin{definition}[Head Error]
\noindent{\textit{\textbf{Localizing Head Error.}}}
%Otherwise, $g_{head}(e_1) = g_{head}(e_2) = c_0 \neq f(x)$, suggesting that the embedding computed by $f_{enc}$ and mapped to the VLM's representation space via $r_{map}$ allows the VLM head to output the correct label, thus the error is in $f_{head}$; we call it \textit{head error}.
If $e_1$ and $e_2$ lead to the same zero-shot classification outputs, i.e., $g_{head}(e_1) = g_{head}(e_2)$, it suggests that the embedding computed by $f_{enc}$ and mapped to the VLM's representation space via $r_{map}$ allows the VLM head to output the correct label, thus the error is in $f_{head}$; we call it \textit{head error}.
%\end{definition}

For example, consider the \textit{ship} images on the left of Fig.~\ref{fig:enc_head_errs} that are mislcassified by ResNet18. The one on the left is misclassified due to the encoder error because $g_{head}(e_2)$ (i.e., CLIP) is \textit{ship} but $g_{head}(e_1)$ (i.e., CLIP via $r_{map}$) is \textit{frog}. 
The one on the right is misclassified due to the head error because $g_{head}(e_2)$ (i.e., CLIP) and $g_{head}(e_1)$ (i.e., CLIP via $r_{map}$) are both \textit{ship} but the ResNet18 output is \textit{dog}.
%\nina{If we have space, I would frame these as definitions (or highlighted somehow) as these are basic notions: encoder and head errors.}. %\caroline{added some sentences about Fig.~\ref{fig:enc_head_errs}} %\divya{maybe we could move these details to 4.3.2 , where we refer to Fig 4? }\caroline{I feel like these examples help with understanding the definition of encoder/head error}

By checking RIVAL-10 test images misclassified by ResNet18, we categorized 61 images as encoder errors (see Fig.~\ref{sfig:truck_enc} for the summary heatmap of misclassified \textit{truck} images) and 84 images as head errors (see Fig.~\ref{sfig:truck_head} for the summary heatmap for the summary heatmap of misclassified \textit{truck} images) respectively. Fig.~\ref{fig:enc_head_errs} shows examples of encoder and head errors identified by our technique. 

\subsubsection{Validating Localization with Mutations.} 
%\subsubsection{Error Localization} %\caroline{summary of this paragraph: we use a mutation-based approach to demonstrate encoder and head error. mutation in encoder [resp. head] led to a significant increase in No. encoder [resp. head] errors. Additionally, with an alternative decomposition, we can localize errors even more, e.g., with residual block 3. }

%\ravi{Section4.3.1 is also about error localization, so I renamed this subsubsection}

%Application of the above technique on the test inputs with ground-truth truck that are misclassified by ResNet18, we categorize 61 as encoder errors and 84 as head errors respectively.

%We would like to use ground-truth based summary heatmaps to validate this categorization. We expect that for inputs localized as encoder errors, the corresponding embedding vectors would not satisfy the strength predicates relevant to the ground-truth label, while the embedding vectors for the head errors would satisfy the relevant strength predicates.

%Show the corresponding heatmaps for the 61 errors and 84 head errors. PUT pictures for ENC and HEAD errors.
To validate our technique for error localization, we employ a mutation-based approach by manually introducing errors in the encoder or the head of ResNet18 by randomizing the weights of a small set of neurons. 
If our technique is valid, then by introducing errors in the encoder, the localization should result in statistically more encoder errors than head errors, and vice versa.
%\nina{It feels to me that we need to explain what exactly we expect to evaluate using mutations.} 
From ResNet18, we created two different mutated models, one with randomized weights for two neurons in each convolutional layer in the encoder, and one with randomized weights introduced only in the final classification layer, i.e., in the head. From row 2 of Tbl.~\ref{tab:enc_head_errors}, we can see that introducing mutations in the encoder resulted in significantly more encoder errors than head errors, as expected. Similarly, from row 3, mutations in the head resulted in significantly more head errors than encoder errors, as expected. 
%From row 2 of Tbl.~\ref{tab:enc_head_errors}, we can see that compared to row 1 for the original ResNet18, the number of encoder errors, identified by our localization technique, significantly increased \divya{compared to what?}\caroline{added} after introducing mutations in the encoder. Similarly, shown in row 3 of Tbl.~\ref{tab:enc_head_errors}, head errors identified by our localization technique significantly increased after mutations in the head. 
%\divya{If I understand correctly, we want to say that in row 2 , our technique identifies more encoder errors than head errors which is in alignment with the ground-truth since the mutation is only in the encoder. It is the reverse in row 3, which is also in alignment with the ground-truth. Is this correct?} \caroline{yes, I reworded these sentences a bit}
This suggests that our localization approach, although not perfect, can be useful in localizing the errors either in the encoder or the head.%}the number of encoder and head errors can indicate the location of errors in the vision model. 
% \caroline{discuss the reason for increasing head error when encoder is mutated and the other way. head is dependent on an encoder? more fine-grained localization is required?}

We attempt to determine if our localization approach can perform a more precise layer-wise localization. %A more precise localization can be conducted with two different encoder head decompositions of the same vision model. 
For example, to localize errors specifically in Residual Block 3 as shown in Fig.~\ref{fig:resnet18-decomp}, we can consider an alternative decomposition for ResNet18 by moving Residual Block 3 from the encoder to the head. %Now, the encoder contains the initial layers, Residual Blocks 0, 1, 2, and the head contains layers from Residual Block 3 on. 
In this case, mutations introduced specifically in Residual Block 3 would be encoder errors with the original decomposition, but head errors with the alternative decomposition. 
Since all Residual Blocks contain convolutional layers, to obtain an accurate $r_{map}$, we added average pooling to reduce the dimensionality of the output of Residual Block 2 before the mapping to CLIP embedding space\footnote{The resulting mapping has MSE of 1.128 and $R^2$ of 0.749, comparable with mapping obtained for the original decomposition}. %\caroline{should we discuss limitations of mapping to CLIP somewhere earlier (like background?)} 
%\susmit{Counts in Table 1 are good but they are missing the containment information. Are all 4271 reported encoder errors in Mutation in Encoder contained in reported head error in Mutation in Head? Another way to look at it would be to report false positive and false negative numbers.} \caroline{Thank you for the suggestion! Sorry I'm not sure I understand completely. Mutation in the head and encoder resulted in two different models, thus the errors are different, I am not sure if this is what you mean and I am not sure what would be the containment information in this case. For false positive/negative numbers, do you mean whether a misclassification was indeed encoder/head error? We don't really have the ground truth for this so we don't have these numbers. We can validate encoder/head error with heatmaps, encoder errors would cause the predicate to look very different. I clarified this in 4.3.3, please check. thank you. }

%\divya{[Suggestion] The last row of Tbl.~\ref{tab:enc_head_errors} shows the number of errors identified as encoder and head errors for the original and alternate decompositions respectively. Counter-intuitively, we find that irrespective of the buggy layer being present as part of the encoder or the head, the number of errors identified as head errors are more than encoder errors. However, the number of encoder errors with the original decomposition is more than the alternate decomposition, indicating a shift in the location of the bug. This highlights the potential of our algorithm with different encoder-head decompositions to precisely locate the buggy layer. However, we leave more detailed evaluation of this for future work.}

The bottom row of Tbl.~\ref{tab:enc_head_errors} presents the number of encoder and head errors with the original and alternate decomposition. Surprisingly, we observe that regardless of the location of the mutation, regardless of whether the mutation is in the encoder or the head, the number of head errors exceeds encoder errors. At the same time, the original decomposition yields more encoder errors compared to the alternate decomposition, indicating a shift in the location of the mutation. This underscores the potential of employing different encoder-head decompositions for precise layer-wise error localization. %Nonetheless, we leave a more comprehensive evaluation addressing the increase in head errors as future work.
%\nina{Do we need last sentence? This is the second time we say that we leave smth to as  future work in evaluation}\ravi{I think we should remove the sentence}
%From the last row of Tbl.~\ref{tab:enc_head_errors}, we can see that around 800 encoder errors become head errors when we switch from the original decomposition to the alternative decomposition, indicating errors specifically located in Residual Block 3. 
%However, counter-intuitively, regardless of the location of the mutation, the number of head errors significantly increased. 
%We noticed that mutation in one location can also increase errors in another location, e.g., the increase in head errors after mutating the encoder. More fine-grained and detailed analysis is required for more precise localization and repair. 


%\caroline{Reason for the increase in head errors?}
%Similar to before, shown on the right side of Tbl.~\ref{tab:enc_head_errors}, the difference in decomposition does affect the localization of errors in the encoder and head, as mutations in the encoder and head led to a significant increase in the number of encoder and head errors. 
%in order to obtain an accurate mapping before mapping the embedding to CLIP space. 

%Intuitively, given a misclassified input image $x$, we consider the error to be either 1) in the image encoder $f_{enc}$ if the embedding of this image does not correspond to the actual features in the image, e.g., wheels in the images incorrectly mapped to the embedding space of beaks, or 2) in the classification head $f_{head}$ if the image is encoded to the correct space, but the head outputs the incorrect label, e.g., incorrectly classifying an embedding of beaks as a truck which does not have beaks. 

%Given input $x$ with ground truth $c_0 \in C$ such that $f(x)\neq c_0$ (vision model misclassifies) and $g(x) = c_0$ (VLM does not misclassify), 
%let $e1 = r_{map}(f_{enc}(x))$ refer to the embedding of $x$ mapped to the VLM embedding space, $e2 = g^{img}_{enc}(x)$ refer to the embedding of $x$ directly produced by the VLM. The error is in $f_{enc}$ if $g_{head}(e1) \neq g_{head}(e2)$, and in $f_{head}$ otherwise. 

%We want to determine if the bug is located in the ENC or HEAD? Can be followed with repair or fine-tuning of the either encoder or header or a specific layer.
%{\it FL results for (i) mis-classified in-dist inputs, (ii) adv , (iii) natural perturbations, (iv) poison  \blue{added, see Tbl.~\ref{tab:enc_head_errors}}\it}
%Explain ENC or Head errors.
%The respective GT heatmaps for ENC and HEAD errors serve as validation for the FL results.

%Experiment:
%\begin{itemize}
%    \item decomposition used
%    \item Mutation-based approach: introducing errors in different parts of the model (head, enc or a specific part using two decompositions)
%    \item check the number of errors in the encoder or head
%    \item use heatmaps to validate: part with errors would show more random heatmaps
%\end{itemize}

%Results we have: (detecting error in enc or head) resnet18, resnet50, vit (soon); (layerwise with two decomposition) resnet18 



\begin{table}[t]
    \centering
    \caption{Number of encoder and head errors found through error localization for all images in the test set. }
    \label{tab:enc_head_errors}
    \scalebox{0.82}{
    \begin{tabular}{|c|>{\columncolor{tuftsblue!15}}c|>{\columncolor{turquoisegreen!20}}c|}
        \hline
        %\multirow{ 2}{*}{Mutation location}
        %& \multicolumn{2}{|c|}{Original decomposition} & \multicolumn{2}{|c}{Alternative decomposition} \\
        %\cline{2-5}
        Mutation location& \# encoder error & \# head error \\%& \# enc error & \# head error\\
         \hline
         No mutation (original ResNet18) & 61 & 84 \\%& 80 & 65 \\
         \hline
         Mutation in Encoder & 4271 & 405 \\%& 3361 & 1305\\
         \hline
         Mutation in  Head & 101 & 4571 \\%& 525 & 4147\\
         \hline
         Mutation in Residual Block 3 & \shortstack{1183 (orig decomp)\\ 438 (alt decomp)} & \shortstack{3064 (orig decomp)\\ 3809 (alt decomp)}  \\%& 438 & 3809 \\
         \hline
    \end{tabular}}
    
\end{table}

%{\it Differential GT Heatmap for in-dist ENC errors \blue{added, see Fig.~\ref{fig:fl}, in both cases, the heatmap looks like correctly classified cats but relevant concepts are not detected}\it}
\begin{figure*}[t]
    \centering
    \begin{subfigure}[t]{0.22\linewidth}
        \centering
        \includegraphics[width=\linewidth]{heatmaps/decomp/resnet18_1_class_truck_enc_error_gt.png}
        \vspace{-0.25in}
        \caption{With mutated encoder. }
        \label{sfig:fl_enc}
    \end{subfigure}
    \hspace{0.1in}
    \begin{subfigure}[t]{0.22\linewidth}
        \centering
        \includegraphics[width=\linewidth]{heatmaps/decomp/resnet18_2_class_truck_enc_error_gt.png}
        \vspace{-0.25in}
        \caption{With mutated head.}
        \label{sfig:fl_head}
    \end{subfigure}
    \hspace{0.1in}
    \begin{subfigure}[t]{0.22\linewidth}
        \centering
        \includegraphics[width=\linewidth]{heatmaps/decomp/resnet18_3_class_truck_head_error_gt.png}
        \vspace{-0.25in}
        \caption{With mutated Residual Block 3 using the original decomposition (mutations in the encoder).}
        \label{sfig:fl_rb}
    \end{subfigure}
    \hspace{0.1in}
    \begin{subfigure}[t]{0.22\linewidth}
        \centering
        \includegraphics[width=\linewidth]{heatmaps/decomp/resnet18_1_3_class_truck_enc_error_gt.png}
        \vspace{-0.25in}
        \caption{With mutated Residual Block 3 using the alternative decomposition (mutations in the head).}
        \label{sfig:fl_rb2}
    \end{subfigure}
    \vspace{-0.1in}
    \caption{Ground-truth summary heatmaps for images with ground truth \textit{truck} for various mutated ResNet18 models. The red outline indicates relevant strength predicates for class \textit{truck}. }
    \label{fig:fl}
\end{figure*} 




\subsubsection{Validating Localization and Analyzing Errors with Heatmaps} 
%\caroline{summary of this paragraph: heatmaps can be used to verify encoder vs head errors. for gt truck images, if relevant strength predicates are sat, encoder is correct, error is likely in head, else, error is likely in the encoder }

With semantic heatmaps, we can visualize and validate localization results and understand the reasons for failure. Heatmaps show the satisfaction of the strength predicates by the output of the encoder, i.e., the image embedding. %Therefore, with encoder errors, the satisfaction of strength predicates would be different than expected in ground truth, e.g., an inaccurate embedding of truck images would not satisfy relevant strength predicates for trucks. If the errors are only in the head, the satisfaction of strength predicates would be similar to ground truth. 
For \textit{truck} images misclassified by the original ResNet18, from Fig.~\ref{sfig:truck_enc}, we can observe that, compared to correctly classified images in Fig.~\ref{sfig:correct_truck}, a few relevant strength predicates have lower satisfaction probability, e.g., $text>patterned$, %$wheels>tail$, $wheels>patterned$,
as well as the ones involving relevant concepts $wheels$ and $tail$;  
%\divya{looks like all relevant strength predicates with wheel as con1, or tail as con2 have lower satisfaction probabilities} \caroline{added in the text} , 
and several non-relevant strength predicates have higher satisfaction, e.g., $ears>mane$, indicating encoder errors. On the other hand, Fig.~\ref{sfig:truck_head} highly resembles Fig.~\ref{sfig:correct_truck}, suggesting the images are correctly encoded and thus the errors are in the head.
%\divya{ maybe we should move the above discussion about the heatmaps to 4.3.3?} \caroline{moved}

Next, to validate localization and further analyze failures of the mutated ResNet18 models, we constructed ground-truth summary heatmaps for images with ground truth truck (Fig.~\ref{sfig:fl_enc}-\ref{sfig:fl_rb2}). We can see in Fig.~\ref{sfig:fl_enc}, with the mutated encoder, many relevant strength predicates for trucks have low satisfaction probability, indicating errors in the image embedding as expected. Specifically, predicates involving \textit{wheels} and \textit{text} have the lowest satisfaction probability, suggesting the encoder is not identifying these specific concepts from the input images. However, with the mutated head, as shown in Fig.~\ref{sfig:fl_head}, relevant strength predicates are still satisfied with high probability, indicating errors are more likely to be in the classification head rather than the encoder, as predicted. For mutated Residual Block 3, with the original decomposition, it is part of the encoder, thus Fig.~\ref{sfig:fl_rb} shows decreased satisfaction probability in a few relevant strength predicates, e.g., $wheels>tail$ and $text>hairy$; with the alternative decomposition, it is part of the head, thus Fig.~\ref{sfig:fl_rb2} shows most relevant predicates are still satisfied with high probability. 

%\caroline{these are future directions?}
%Can help focus testing and repair; generate test inputs that satisfy the violated predicates, repair the encoder to satisfy the violated predicates for the failing inputs. 


\begin{figure*}[t]
    \centering
    \begin{subfigure}[t]{0.22\linewidth}
        \centering
        \includegraphics[width=\linewidth]{heatmaps/decomp/pgd_truck.jpg}
        \vspace{-0.25in}
        \caption{Ground-truth heatmap for all perturbed images (PGD with $l_{\infty}$). }
        \label{sfig:rf_pgd}
    \end{subfigure}
    \hspace{0.05in}
    \begin{subfigure}[t]{0.22\linewidth}
        \centering
        \includegraphics[width=\linewidth]{heatmaps/decomp/pgd_diff_truck.jpg}
        \vspace{-0.25in}
        \caption{Differential heatmap displaying the absolute difference between Fig.~\ref{sfig:correct_truck} and Fig.~\ref{sfig:rf_pgd}.}
        \label{sfig:rf_diff}
    \end{subfigure}
    \hspace{0.05in}
    \begin{subfigure}[t]{0.22\linewidth}
        \centering
        \includegraphics[width=\linewidth]{heatmaps/decomp/pgdl2_truck.jpg}
        \vspace{-0.25in}
        \caption{Ground-truth heatmap for all perturbed images (PGD with $l_2$). }
        \label{sfig:rf_pgd2}
    \end{subfigure}
    \hspace{0.05in}
    \begin{subfigure}[t]{0.22\linewidth}
        \centering
        \includegraphics[width=\linewidth]{heatmaps/decomp/pgdl2_diff_truck.jpg}
        \vspace{-0.25in}
        \caption{Differential heatmap displaying the absolute difference between Fig.~\ref{sfig:correct_truck} and Fig.~\ref{sfig:rf_pgd2}.}
        \label{sfig:rf_diff2}
    \end{subfigure}
    \vspace{-0.1in}
    \caption{Heatmaps for identifying robust and non-robust features against Projected Gradient Descent (PGD) attack (both $l_{\infty}$ and $l_2$). All heatmaps consider images with ground truth \textit{truck}. The black outline shows robust strength predicates where the absolute difference in satisfaction probability $\leq0.05$. The red outline indicates relevant strength predicates for class \textit{truck}.}
    \label{fig:rf}
\end{figure*}   



%\subsection{Application 3: Identification of Robust and Non-robust Strength Predicates}
\subsection{Application 3: Debugging for Robustness}
%Identification of Robust and Non-robust Strength Predicates}
\label{subsec:robust_feat}
%\caroline{summary of this paragraph: we can identify features (that are the satisfaction of strength predicates) robust in the presence of adv perturbations. we show heatmaps for a perturbation resnet18 is robust to (pgd l2) and one it is not (pgd $l_{\infty}$)}

%Vision models can be vulnerable to adversarial perturbations, i.e., small perturbations in the inputs can cause misclassification~\cite{Szegedy2014IntriguingPO}, thus robustness analysis is necessary for risk assessment of vision models. Concept-based analysis allows us to extend analysis beyond accuracy and identify strength predicates that can and cannot be robustly satisfied by the vision models in the presence of adversarial perturbations, which is important for understanding the predictability and adaptability of the vision models. A strength predicate is robust against a perturbation if the satisfaction probability (that is $>0$) remains the same before and after applying the perturbation, and non-robust otherwise. 
%\corina{do we explain anywhere why finding robust/non robust features is important? perhaps in intro?}

%\divya{In the section below, shouldn't we be referring to Figures 3a for the heatmaps for non-perturbed truck images? Fig 3b is the subset of truck images which are also correctly classified.}\caroline{yes, corrected}

With ResNet18, Fig.~\ref{fig:all_truck}  shows the ground-truth summary heatmap obtained with all original \textit{truck} images without any perturbations, and Fig.~\ref{sfig:rf_pgd} shows the heatmap obtained with all \textit{truck} images perturbed with Projected Gradient Descent (PGD) (perturbation radius $ \epsilon=\frac{8}{255}$)~\cite{MadryMSTV18}. ResNet18 has a $0\%$ accuracy on all perturbed images, i.e., not robust against the $l_{\infty}$ PGD attack. This is also evident in Fig.~\ref{fig:all_truck} and Fig.~\ref{sfig:rf_pgd}---the satisfaction of most strength predicates is affected by the perturbation. By visualizing the absolute difference between these two heatmaps (see Fig.~\ref{sfig:rf_diff}, lighter green indicates a smaller difference), we can identify a small set of strength predicates that remained constant, i.e., with absolute difference $\leq 0.05$, that are robust predicates, e.g., %$ears>beak
$rectangular>horns,~long>ears$, and the rest are non-robust predicates, e.g., $wheels> tail,~%rectangular>tail$
metallic > long-snout$. Notice that the majority of all relevant strength predicates for \textit{trucks} are not robust, suggesting ResNet18 is not robust against $l_{\infty}$ PGD.
%\divya{mention some more robust and non-robust features}. 
Additionally, considering the $l_{2}$ PGD attack ($\epsilon=\frac{8}{255}$), ResNet18 is robust---it has a $96.3\%$ accuracy on all perturbed images. In addition to high accuracy, we can validate using the heatmap obtained for all \textit{truck} images perturbed with $l_{2}$ PGD attack(Fig.~\ref{sfig:rf_pgd2}) as well as the differential heatmap between Fig.~\ref{fig:all_truck} and Fig.~\ref{sfig:rf_pgd2}. We see that ResNet18 can robustly satisfy all of the strength predicates. 
%In this case, all the non-robust predicates have satisfaction probability $0$ before and after the perturbation. \ravi{i dont understand why these are being called non-robust? Isnt a predicate non-robust only if there is a big change in satisfaction probability after perturbation?} 
%\divya{point out non-robust features if any. Some irrelevant predicates have a large difference example floppy-ears - mane, rectangular - wheels. Mention that these do not impact model output for truck.} 
By analyzing model robustness through concepts, we assign meaning to statistical results, allowing us to better understand the effects of the adversarial perturbations, and thus allowing developers to design more meaningful detectors and attacks.

Additionally, this experiment highlights that most adversarial examples get misclassified due to encoder errors. 
While the encoder of ResNet18 is nearly accurate for in-distribution inputs, adversarial perturbations can lead to incorrect encoding as suggested by the non-robust features. Such insights can facilitate re-training or repair efforts by directing attention to the encoder and the specific non-robust strength predicates.


%Tail is a concept, $tail > metallic$ is a feature. 
%Identify invariant properties. 
%Can help re-training with focus on the non-robust features. 

%Experiment:
%\begin{itemize}
%    \item plot heatmaps w.r.t. ground truth before and after perturbations, 
%    \item highlight features ``preserved'' (diff $\leq threshold$) 
%\end{itemize}

%\blue{Results are shown in Fig.~\ref{fig:rf}.}

%Results we have: (adv) pgd, fab, fgsm, pgdl2, mix, (natural) brightness%, (poison) gradient matching, \red{can run more if needed}

\begin{figure*}[t]
    \centering
    \begin{tabular}{ccc}
    \begin{subfigure}[t]{0.3\linewidth}
        \centering
        \includegraphics[width=\linewidth]{heatmaps/decomp/pgd_truck_outout.jpg}
    \vspace{-0.25in}
    \caption{Output-label summary heatmap for perturbed images classified as \textit{truck}.}
    \label{sfig:detect_pgd}
    \end{subfigure} &
    \begin{subfigure}[t]{0.3\linewidth}
        \centering
        \includegraphics[width=\linewidth]{heatmaps/decomp/correct_pgd_truck_bin.jpg}
    \vspace{-0.25in}
    \caption{Binarized heatmap of correctly classified clean images of \textit{trucks} (binarized Fig.~\ref{sfig:correct_truck}). }
    \label{sfig:detect_c}
    \end{subfigure}&
    \begin{subfigure}[t]{0.3\linewidth}
        \centering
        \includegraphics[width=\linewidth]{heatmaps/decomp/pgd_truck_bin.jpg}
        \vspace{-0.25in}
        \caption{Binarized heatmap of perturbed images classified as \textit{truck} (binarized Fig.~\ref{sfig:detect_pgd}). }
        \label{sfig:detect_pgd_b}
    \end{subfigure}\\
    \end{tabular}
    \vspace{-0.1in}
    \caption{Heatmaps used for runtime detection of adversarial inputs with ResNet18. Adversarial inputs generated with $l_{\infty}$ PGD attack, $\epsilon=\frac{8}{255}$. Fig.~\ref{sfig:detect_c} and Fig.~\ref{sfig:detect_pgd_b} binarized with threshold $0.6$. Red outlines indicate relevant strength predicates for class \textit{truck}. }
    \label{fig:fl}
    %\vspace{-0.1in}
\end{figure*} 

\begin{table*}[t]
    \centering
    \caption{Accuracy for detecting adversarial inputs vs clean inputs with heatmaps for all images in the test set. For each class $c$, we have about 500 clean images with ground truth $c$ and 500 perturbed images that are labeled by ResNet18 as $c$. Each cell contains ($a_p$, $a_n$) where $a_p$ is the percentage of perturbed images correctly detected as adversarial inputs ($IoU_p > IoU_n$), and $a_n$ percentage of clean images correctly detected ($IoU_p \leq IoU_n$). $\epsilon$ is $\frac{8}{255}$ for all experiments.}
    \label{tab:adv_acc}
    \vspace{0.05in}
    \begin{tabular}{cccccc}
    \toprule
        & \shortstack{PGD $l_{\infty}$} & \shortstack{FAB $l_{\infty}$} & \shortstack{FGSM $l_{\infty}$} & \shortstack{PGD $l_{2}$} & \shortstack{Mixture}\\
         \midrule
         \textit{truck} & (0.943 , 0.497) & (0.961 , 0.647) & (0.930 , 0.887) & (0.779 , 0.256) & (0.793 , 0.529)\\
        \textit{car} & (0.977 , 0.522) & (0.990 , 0.577) & (0.932 , 0.730) & (0.893 , 0.112) & (0.936 , 0.653)\\
        \textit{plane} & (0.913 , 0.627) & (0.952 , 0.694) & (0.950 , 0.805) & (0.890 , 0.127) & (0.944 , 0.725)\\
        \textit{ship} & (0.886 , 0.732) & (0.901 , 0.757) & (0.941 , 0.929) & (0.718 , 0.301) & (0.901 , 0.783)\\
        \textit{cat} & (0.479 , 0.937) & (0.938 , 0.802) & (0.915 , 0.706) & (0.866 , 0.146) & (0.535 , 0.800)\\
        \textit{dog} & (0.787 , 0.593) & (0.960 , 0.618) & (0.950 , 0.600) & (0.880 , 0.137) & (0.813 , 0.526)\\
        \textit{equine} & (0.552 , 0.871) & (0.901 , 0.819) & (0.903 , 0.866) & (0.872 , 0.161) & (0.771 , 0.707)\\
        \textit{deer} & (0.921 , 0.614) & (0.939 , 0.720) & (0.947 , 0.856) & (0.867 , 0.152) & (0.939 , 0.675)\\
        \textit{frog} & (0.865 , 0.658) & (0.910 , 0.634) & (0.940 , 0.716) & (0.904 , 0.117) & (0.856 , 0.627)\\
        \textit{bird} & (0.795 , 0.558) & (0.964 , 0.794) & (0.962 , 0.640) & (0.972 , 0.034) & (0.816 , 0.613)\\
        \hline
        Total & (0.810 , 0.663) & (0.941 , 0.711) & (0.937 , 0.764) & (0.864 , 0.154) & (0.830 , 0.681)\\
         \bottomrule
         \multicolumn{5}{l}{*All numbers are rounded.}
    \end{tabular}
    \vspace{-0.1in}
\end{table*}

\subsection{Application 4: Runtime Detection of Adversarial Inputs}
\label{subsec:adv_detect}
%\caroline{Summary of this paragraph: run time detection can be done by comparing each single-input heatmap with summary heatmaps of 1) correctly classified original images of a class; 2) perturbed images misclassified to this class. The comparison can be done by simply binarizing summary heatmaps with a threshold, and using IoU to determine whether each single-input heatmap is more similar to heatmap 1) or heatmap 2). Using CLIP directly can give more accurate results, but CLIP is too expensive for runtime detection. }

%\corina{do we explain anywhere what adversarial inputs are and why it is important to detect them??}

So far, we have primarily relied on the ground-truth summary heatmaps for interpreting model behaviour. When ground truth information is unavailable, e.g., during runtime, we can utilize output-label summary heatmaps for analysis, for instance, enabling runtime detection of adversarial inputs. As we observed before, adversarial perturbations lead to encoder errors. Therefore, with output-label summary heatmaps of a particular class, the relevant strength predicates would appear satisfied. 
%Intuitively, perturbations can affect the encoding of concepts in the inputs, therefore, heatmaps for non-perturbed images of one class would be different from heatmaps for perturbed images classified to the same class.
%Adv detectionL since adv perturbations lead to encoder errors, when look at output based heatmaps for a label, the relevant predicate gets satisfied by both miusclassifie and correctly classified; but the not-relevant are different. Since they were mapped from other classes, giving random satisfaction rate. We zoom in on this, thus we use single-output and then …. Reason this relevant seems same with perturbat, previously, adv lead to lots of encoder errors.
For example, consider PGD $l_{\infty}$  attack ($\epsilon=\frac{8}{255}$); Fig.~\ref{sfig:detect_pgd} shows the summary heatmap for all perturbed images misclassified to \textit{truck} by ResNet18. Most relevant strength predicates for \textit{trucks} are satisfied since these images are classified as \textit{trucks}. However, since these images are incorrectly mapped to \textit{trucks} from other classes, the strength predicates not relevant to \textit{truck} but that are relevant for other classes, show a more different and random satisfaction rate. Zooming in on this for adversarial detection, for each input, we identify such differences in its single-input heatmap.%\divya{single-input heatmap} 
%Compared to Fig.~\ref{sfig:rf_c}, the satisfaction of most strength predicates is affected by the perturbation and differs from that of non-perturbed images. 
%We demonstrate that adversarial inputs can be detected during runtime by identifying such differences.


First, for each output class, we construct a ground-truth summary heatmap with all clean images (i.e., a clean heatmap as in Fig.~\ref{sfig:correct_truck} for \textit{truck}) 
%\ravi{Do we conside ground-truth heatmaps or output heatmaps for clean images? Seems like we should consider output heatmaps} 
and a output summary heatmap with all adversarial inputs generated during offline analysis (i.e., a perturbed heatmap as in Fig.~\ref{sfig:detect_pgd} for \textit{truck}). Then, for each input encountered during runtime with output class $c$, this input is considered adversarial if its single-input heatmap is more similar to the perturbed heatmap than the clean heatmap of class $c$, and clean otherwise. To determine the similarity between a single-input heatmap and the above summary heatmaps,
%\susmit{is summary over all of training data - different inputs have different heatmaps}\caroline{addressed}, 
we first binarize the summary heatmap with a threshold $t$ %\susmit{some insight into selection of t would be useful}\caroline{added after this sentence, please check} 
to highlight strength predicates with high satisfaction probabilities, i.e., $1$ if satisfaction probability $\geq t$, and $0$ otherwise. 
The value of $t$ should be sufficiently high to capture the primary differences between clean and perturbed heatmaps while avoiding the inclusion of small values that are predicates satisfied by only a small set of images. In our experiment, we set 
$t=0.6$, which resulted in the highest detection accuracy.
The binarized clean heatmap (binarized Fig.~\ref{sfig:correct_truck}) is shown in Fig.~\ref{sfig:detect_c}; and the binarized perturbed heatmap (binarized Fig.~\ref{sfig:detect_pgd}) is shown in Fig.~\ref{sfig:detect_pgd_b}, with $t=0.6$. Then we compute Intersection over Union (IoU) as the similarity metric, between each single-input heatmap and the binarized summary heatmaps; we use $IoU_p$ for similarity with the the binarized perturbed heatmap, and $IoU_n$ for similarity with the binarized clean heatmap. An input with $IoU_p > IoU_n$ suggests it is adversarial, and clean otherwise.


To demonstrate runtime detection of adversarial inputs, 
%we considered common adversarial perturbations 
we constructed sets of perturbed inputs (all with $\epsilon=\frac{8}{255}$) using common adversarial attacks such as 
PGD (both $l_{\infty}$ and $l_2$)~\cite{MadryMSTV18}, FGSM ($l_{\infty}$)~\cite{Szegedy2014IntriguingPO}, FAB ($l_{\infty}$)~\cite{croce2020minimally}, and a random mixture of all the above. In Tbl.~\ref{tab:adv_acc}, we show the accuracy of identifying perturbed from clean images per class. Overall, we were able to achieve high accuracy for most classes and most perturbations with a simple similarity metric. This suggests our heatmaps have the potential for more precise runtime detection. For PGD $l_2$ with lower accuracy in Tbl.~\ref{tab:adv_acc}, as we showed in Sec.~\ref{subsec:robust_feat}, ResNet18 is robust against PGD $l_2$ with high robust accuracy, thus the perturbed and clean heatmaps are too similar for differentiating adversarial inputs. Additionally, we noticed that adversarial attacks affect different classes differently---classes with lower accuracy have more similar perturbed and clean heatmaps,
%\ravi{this contradicts the previous statement that suggests that if the model performance is similar for clean and adv inputs, i.e., model is robust, then heatmaps are similar},
suggesting the model is more robust for some classes of inputs than others. 
%Overall these results suggest that our adversarial detector works better when the model is less robust since the clean and adversarial heatmaps are very similar in these cases.

%we only used images clip correctly classified. Attack works differently for different classes: classes with low accuracy have similar heatmaps between original and perturbed data (model is robust).
Note that VLMs such as CLIP can themselves be deployed as runtime detectors to catch inputs misclassified by the vision model. CLIP has robust accuracy $0.982$ against PGD $l_{\infty}$, $0.984$ against FAB, $0.973$ against FGSM, and $0.984$ against PGD $l_{2}$, all of which are higher than detection accuracy with semantic heatmaps. However, foundation models such as CLIP are too computationally heavy to be deployed during runtime, while our heatmaps can be precomputed, only the single-layer linear aligner $r_{map}$ is required during runtime, which is more desirable for analysis during runtime. 



%However, our concept-based detection technique is more desirable due to the following reasons; (i) Foundation models such as CLIP are heavy-weight to deploy at runtime, (ii) The zero-shot classification of CLIP is not 100\% so the runtime ``oracle" may be wrong. On the other hand, the concept-based heatmaps are built only using instances on which CLIP is 100\% accurate, further they employ finer-grained information in terms of concepts. Hence this technique has the potential to have more precise detection


%We describe offline analysis of r such inputs.
%\blue{also show results for directly using CLIP}
%CLIP acc:
%\begin{itemize}
%    \item pgd: 0.9820279984865683
%    \item fab: 0.9841089670828603
%    \item fgsm: 0.9729474082482028
%    \item pgdl2: 0.9844873250094589
%    \item mix: 0.9752175558077941
    %\item brightness: 0.14812712826333713
%\end{itemize}



%\subsubsection{Adv data}

%Experiment \blue{see Fig.~\ref{fig:adv} and Tbl.~\ref{tab:adv_acc} (using images that CLIP correctly classified)}:
%\begin{itemize}
%    \item plot heatmaps w.r.t. model output before and after perturbations
%    \item detection by comparing IoU with original heatmap and perturbed heatmaps
%    \item best results achieved together with robust features
%\end{itemize}

%Additional observations: 
%\begin{itemize}
    %\item CLIP is not robust to natural perturbations like brightness: images misclassified by the model are also misclassified by CLIP
    %\item Attack works differently for different classes: classes with low accuracy have similar heatmaps between original and perturbed data (model is robust). 
    %\item CLIP is not robust to natural perturbations
    %\item natural perturbations can be detected (heatmaps are quite different), but detecting misclassification like adv is harder
%\end{itemize}

%Results we have: (adv) pgd, fab, fgsm, pgdl2, mix, (natural) brightness





%\subsubsection{Poisoned data}
%Previously, people showed that for poisoned data, the model uses different features, and different groups of neurons are activated than the original data. We can assign meaning to these features, verify the assumption of previous work and give explanations of model behaviour. 


%\subsection{Future Directions}
%\caroline{summary of future work: repair, data selection for retraining, adv detection, etc. }
%\caroline{summary of discussion: in error localization, introducing errors in head also increased encoder errors, further analysis is required; the clip version we used is not robust to natural perturbations, e.g., brightness}


%Our results can assist testing and repair of the vision models, and enable more localized repair. 

%in localization, other error increases 

%Bugs localization and visualization with heatmaps can help with testing and repair of the vision models, including test generation focusing on violated predicates, and localized repair.





==> sections/framework.tex <==
\section{Framework with VLM}
\label{sec:framework}

\begin{itemize}
    \item Decomposition of HEAD and ENC
    \item Definition of ENC error and HEAD error with VLM
    \item Obtain explanation of errors with $Con_{spec}$
\end{itemize}

==> sections/heatmaps.tex <==
\section{Heatmaps}
\label{sec:heatmaps}

\begin{itemize}
    \item our unified way of looking inside the model, heatmaps capture what the model thinks about the image
    \item constructing heatmaps
    \item validation of heatmaps \red{which figure to use? correct/gt}
\end{itemize}

==> sections/introduction_copy.tex <==
\section{Introduction}
\label{sec:introduction}

%\divya{Divya will add more citations to this section.}


Application of standard practises for offline and online safety assurance, such as testing, debugging, and runtime monitoring is challenging for DNN-enabled systems. This is because, unlike traditional software programs, whose implementation is driven by input-output specifications of behavior, DNNs learn from concrete input-output examples and have an opaque, monolithic, and highly-interconnected structure. It is challenging to interpret the %logical 
% susmit: commented out logical because one could argue DNNs don't do  logical reasoning and many tasks only require statistical reasoning but even that reasoning is opaque unlike say, how one could interpret a Bayesian model implemented using GPs. It is not just logical reasoning but any kind of reasoning that is opaque with DNNs 
reasoning employed by a DNN to make its decisions. For instance, given a set of inputs on which the model fails to produce the expected outputs, it is difficult to explain the reason for this in human-understandable terms, which hinders the debugging process. In fact, even if the model produces the expected output on a given set of inputs, it is not possible to determine if it does so for the right reasons, which is essential to ensure reliability of its performance on unseen inputs. 

Existing techniques for debugging, testing and runtime monitoring typically apply standard approaches from software engineering, such as structural coverage guided testing~\cite{sun2019structural,pei2017deepxplore,odena2019tensorfuzz,usman2023overview} and spectrum-based~\cite{ma2018mode,eniser2019deepfault} as well as mutation-based fault localization~\cite{GhanbariTAR23}. However, it is difficult to make sense of the output artifacts of these activities for DNNs. For instance, a set of neurons marked suspicious %set of neurons executed more often by failing tests than by passing tests, 
does not give us an idea of what exactly is wrong with the logic. 
% Susmit: check to see if this is okay to keep %Divya: Thank you!
It has also been shown in the literature that neurons are  polysemantic and do not capture localized context-free concepts~\cite{sikka2023detecting,sur2023tijo,elhage2022superposition}.
%It does not answer questions such as {\it "Are there any features that the model has not learned correctly?" \it}. 
%Lack of this knowledge 
This inhibits generation of tests that can target the root cause of the problem, beyond the symptoms exposed by the current set of tests. Attribution approaches~\cite{simonyan2014deep,sundararajan2017axiomatic} attempt to identify portions of an input that impact model prediction the most. This can help debug individual tests but does not provide a global understanding of the underlying problem in the model.

\vspace{0.05in}
\noindent
\textit{\textbf{Structure of Vision Models.}} In this work, %\corina{also this is very awkward what do we propose exactly?} 
we propose that it would be more meaningful and effective if activities such as debugging are driven by an abstraction of the DNN logic that promotes interpretability in human-understandable terms. %should be driven an abstraction of the internals of a DNN model, which can enable us to understand {\it what the model is thinking in terms of human-understandable concepts. \it} This abstraction serves to interpret the logic of a DNN model in terms of simple human-understandable terms. Using this interpret-ability as the basis to drive activities such as debugging, can potentially make them more effective and also help obtain more meaningful results. This, in turn, paves way to make more sense of the assurance guarantees provided by these activities and thereby build trust in the system.
%We are driven by the following insights. 
%Unlike the logic-based \divya{maybe remove logic-based? We say in the text below that the head applies logic in terms of concepts.}\ravi{updated below} \corina{maybe just remove unlike the logic  based structure of traditional programs as it seems incorrect} \divya{Ok} structure of traditional programs, 
The architecture of DNNs (specifically those used for vision) is typically composed of an \emph{encoder} followed by a \emph{head}~\cite{pmlr-v80-kim18d,crabbe2022concept,moayeri2023text,Zhou_2018_ECCV}. The encoder is responsible for translating low-level inputs (pixels composing images) into high-level representations in terms of concepts. The head then reasons in terms of these concepts to makes predictions.
The representation space (the latent space of the model after the encoder), therefore, encodes all the high-level concepts that the model has learnt from the examples representative of the domain and can act as an abstraction which aids in interpreting model behavior. However, inferring representations of the concepts learned by a model %(as regions or directions in the latent space) 
is a challenging exercise, typically requiring  manual annotations of inputs with the presence/absence of relevant concepts~\cite{CrabbeS22,KimWGCWVS18,GhorbaniWZK19,Zhou_2018_ECCV,pmlr-v80-kim18d,DBLP:series/faia/YehKR21}. %\corina{here we need a citation}\divya{added TCAV, CAR and some more recent papers.}
%Previous work aims to extract meaningful concept representations, often in the form of directions (of vectors), from the latent spaces of neural networks. In practice, inferring the concept representations learned by a DNN can be challenging, as finding the direction corresponding to a concept requires data that is manually annotated with truth values of concept predicates. It can also be the case that the concepts are entangled and that no such directions exist. 
%Standard practises to ensure safety of systems, such as testing, debugging, runtime monitoring, formal verification so on, require a traceability between high-level domain-specific concepts in which requirements are expressed and the implementation of the software. This is a challenge for systems with DNN-enabled components since unlike in traditional software programs, their implementation is not driven by input-output specifications. DNN models learn from concrete input-output examples and have an opaque, monolithic and highly-interconnected structure. The network inputs are in terms of raw data such as pixels of an image, and not system-level concepts. It is challenging to interpret the logical reasoning employed by a neural network to make its decisions, which in turn hinders the use of the aforementioned standard activities for safety assurance.
%{\bf Divya: give details on some existing methods used for explaining behavior, debugging and runtime monitoring of vision models and their challenges. Give more motivation for using VLMs for these activities. \bf }
%\begin{itemize}
%\item {\bf Notes. To expand \bf} A group of existing techniques for DNN testing, runtime monitoring are black-box [CITE]; utilize high-level features/ simulation parameters but can miss subtle bugs, redundant tests. 
%\item {\bf Notes. To expand \bf} White-box approaches (testing based on structural-coverage [CITE], fault-localization based on test spectrum [CITE], attribution-based approaches[CITE], repair [CITE], runtime-guards for poison/adv detection [CITE]) purely use structural entities of the network such as neurons. DNN structure and implementation is very different software programs therefore traditional software engineering activities cannot be directly applied to a DNN model. Validation of fault-localization or repair is purely based on validation on a separate test set. Attribution has been used to link model outputs to structural entities, and also structural entities to inputs, but difficult to establish traceability to domain-specific concepts. 
%\item {\bf Notes. To expand \bf}existing techniques for concept-based analysis [CITE].previous
%work on concept representation analysis aims to extract meaningful
%concept representations, often in the form of directions (of vectors), from the latent
%spaces of neural networks, that are easy to understand and process. In practice,
%inferring the concept representations learned by a DNN can be challenging, as
%finding the direction corresponding to a concept requires data that is manually
%annotated with truth values of concept predicates. It can also be the case that
%the concepts are entangled and that no such directions exist. 
%\end{itemize}

\vspace{0.05in}
\noindent
\textit{\textbf{VLMs as a Lens.}} Recent work ~\cite{mangal2024conceptbased} explores leveraging vision-language foundation models (VLMs) as a lens to analyze other vision models in terms of human-understandable concepts. VLMs such as CLIP~\cite{pmlr-v139-radford21a}---capable of consuming both images and text as inputs---have been trained on a large body of images accompanied by their textual descriptions and are implicitly aware of high-level concepts describing the images. They offer an exciting opportunity to enable the use of natural language for probing and reasoning about visual data.
% \nina{The part about $Con_{spec}$ seems to be very low-level compared to the rest. I think it will be hard for the reader to understand.} 
% \nina{[Suggestion:] To reason about these high-level concepts and their interactions, a new formal language, $\conspec$, was introduced in ~\cite{mangal2024conceptbased}. It operates over VLM concepts and allows reasoning about any model in terms of these concepts given a proper mapping from its representation space to the VML space.}\divya{Incorporated suggestion.}
%A novel domain-specific logical specification language, $Con_{spec}$, is introduced in ~\cite{mangal2024conceptbased}, that enables experts and developers to express domain knowledge as fine-grained logical predicates in terms of human-understandable concepts. The semantics of the language are in terms of the embedding space of VLMs. Reasoning of other vision models in terms of $Con_{spec}$ is enabled by building an affine map between the image embedding space of the vision-based DNN and the corresponding image embedding space of the VLM. As a consequence, the image representation space of a VLM can serve as a proxy for the representation space of a separate vision-based DNN. 
%
%
% To reason about these high-level concepts and their interactions, a new formal language, $\conspec$, was introduced in ~\cite{mangal2024conceptbased}. It operates over VLM concepts and allows reasoning about any model in terms of these concepts given a proper mapping from its representation space to the VLM space.
% \susmit{We are all FM enthusiasts here and formal is always better, no questions on that :D ... but for other readers - one question here would be why did I need a formal language. Can we make arguments about compositionality here? May be just change ``interaction" to ``composition" and then say, a formal language to describe such compositions? CLIP gets us atomic concepts but composition is part of human-provided spec and we need a formal language to describe that composition. Folks can still ask ``Can just CLIP embeddings of composite specs in natural language suffice and we don't need a formal language?" Some simple empirical evaluation can reject this hypothesis. }
The use of VLMs as a lens is enabled by the recent observation that the representation spaces of vision models and VLMs can be linked to each other~\cite{moayeri2023text}, making it feasible to use the representation space of a VLM for interpreting behavior of vision models.


%In this work, we build on ~\cite{mangal2024conceptbased}, to construct a concept-based abstraction of vision models and use this abstraction to drive explainability, debugging and runtime monitoring activities
%In this work, we leverage the concept-based reasoning enabled by ~\cite{mangal2024conceptbased} to drive explainability, debugging and runtime monitoring activities of vision models. \nina{It feels we need to explain more what we mean by concept-based abstraction. It reads like it is smth similar to concept bottleneck abstraction, so it is not clear what exactly we refer to.}. 
% \nina{[Suggestion to add:] One of the main characteristics of $\conspec$ is that it allows reasoning about relationships between abstract concepts, like one concept being present more strongly than another concept, for a given image. This form of abstract reasoning turned out to be very useful in analyzing DNN models.}\divya{Incorporated.}


% One of the main characteristics of $\conspec$ is that it allows reasoning about relationships between concepts such as one concept ($con_1$) being present more strongly than another concept ($con_2$), for a given image (termed as strength predicates $con_1 > con_2$). %This form of abstract reasoning turns out to be very useful in analyzing DNN models. 
% Previous work ~\cite{mangal2024conceptbased} focuses on the formal verification of properties expressed in terms of strength predicates.
% \susmit{Attempting a rewrite: In practice, concepts often overlap and the presence or absence of a concept in an input is quantitative rather than just Boolean. $\conspec$ recognizes and incorporates this necessity and allows reasoning over one concept ($con_1$) being present more strongly than another concept ($con_2$), for a given input such as an image. The strength predicates  $con_1 > con_2$ in $\conspec$ capture such a nuance and prior work~\cite{mangal2024conceptbased} used this for formal verification.
% %\divya{Thank you for this suggestion , Susmit. Would there be a citation we could use to support the first sentence?} \corina{I think this is based on our own observations we do not need a citation}
% However, it was found that it is not feasible to obtain proofs for most of the strength predicate-based properties.}\corina{I would incorporate this from Susmit}
%\divya{Thank you for this suggestion , Susmit. Would there be a citation we could use to support the first sentence?} \corina{I think this is based on our own observations we do not need a citation}
%However, it was found that it is not feasible to obtain proofs for most of the strength predicate-based properties.
%
In particular, \cite{mangal2024conceptbased} introduced a new formal language, $\conspec$, for writing compositional concept-based specifications about vision classifiers. These specifications relate the presence or absence of concepts in an image to the label predicted by the classifier. However, in practice, concepts often overlap and the presence or absence of a concept in an input is quantitative rather than just Boolean. $\conspec$ recognizes and incorporates this necessity; it allows reasoning over one concept ($con_1$) being present more strongly than another concept ($con_2$) in a given input image by introducing the notion of \emph{strength predicates} (denoted as $con_1 > con_2$). While~\cite{mangal2024conceptbased} focused on the formal verification of vision models with respect to $\conspec$ specifications involving strength predicates, it was found that it is not feasible to obtain proofs for most of these strength predicate-based properties.

\vspace{0.05in}
\noindent
\textit{\textbf{Our Work.}} In this work, we take a statistical approach to analyze neural network behavior in terms of concepts by leveraging the concept-based reasoning enabled by ~\cite{mangal2024conceptbased}. %to drive explainability, debugging and runtime monitoring activities of vision models. 
This allows for more in-depth analysis in a scalable manner, thus paving way to exploring the potential of the {\it concept-based analysis of vision models via VLM \it} paradigm in many more applications. Specifically, we use concept-based analysis to drive explainability, debugging, and runtime monitoring activities for vision models.



%To illustrate concretely, consider a vision model tasked with distinguishing between classes {\it cat, dog, bird, car,} and {\it truck\it}. Relevant concepts for such a domain (identified by domain experts and developers) include concepts such as \textit{metallic}, \textit{wheels} for class {\it truck \it};  \textit{ears}, \textit{tail} for classes \textit{cat} and \textit{dog};  \textit{wings} for class {\it bird \it}; and so on.
To illustrate concretely, consider a vision model tasked with distinguishing between classes {\it cat, bird,} and {\it truck\it}. Relevant concepts for such a domain (identified by domain experts and developers) include concepts such as \textit{metallic}, \textit{wheels} for class {\it truck \it};  \textit{ears}, \textit{tail} for class \textit{cat};  \textit{wings} for class {\it bird \it}; and so on.
%Domain knowledge, in terms of human-understandable concepts, could be expressed using the primitives in the $con_{spec}$ language. Specifically, {\it strength predicates \it} help capture the relationships between concept pairs.  
%For instance, for a vision model tasked with distinguishing between classes like \textit{cat, dog, bird, car,} and \textit{truck}, relevant concepts could be \textit{metallic, ears, wings} and \textit{wheels}. 
%Given an input image, we could probe the model using queries encoded in $Con_{spec}$ such as {\em metallic $\strength$ ears } and {\em wheels $\strength$ wings} which indicates a stronger presence of the concepts, \textit{metallic} and \textit{wheels}, in comparison with other concepts such as \textit{ears} and \textit{wings}, in the representation space of the model for the given input. 
Given an input image of a \textit{truck}, we could probe the model using queries encoded in $Con_{spec}$ such as {\em metallic $\strength$ ears } and {\em wheels $\strength$ wings} to check if the model identifies \textit{truck}-related concepts \textit{metallic} and \textit{wheels} more strongly than concepts \textit{ears} and \textit{wings} in its representation space for the given input. 
%Satisfaction of the aforementioned predicates would indicate that the model was indeed able to identify concepts such as {\it metallic \it} and {\it wheels \it} in the given input image more strongly than the other concepts. 
% \nina{This sentence is not clear. I think what not clear is why we need relations between concepts to determine that `the model potentially encoded the respective concepts'}\divya{addressed.}.
If the model correctly classifies this image as a {\it truck \it} and indeed satisfies these concept-based strength predicates relevant to class {\it truck \it}, it enables the developer to determine that the decision was made for the right reasons, thereby promoting {\it explainability \it}. %satisfaction of the aforementioned concept-based predicates\nina{we need to mention what the relevant concept-based predicates are} \divya{explained in line 132,133.} enables {\it explainability \it}, and helps the developer determine if the decision was taken for the right reasons. 
On the other hand, if the image is mis-classified to a different class, the developer can {\it debug \it} the model by investigating which concept-based strength predicates are violated to obtain an idea of the root cause 
%(in terms of human-understandable concepts) that the model may not have learned correctly. 
(in human-understandable terms) by recognizing the concepts that the model may not have learned correctly. 

%A global understanding of the logic of the model for different scenarios can be obtained by applying the approach to different categories of inputs of interest. Given a set of inputs (such as passing and failing tests, inputs with adversarial and natural perturbations, poisoned inputs so on),  %map the corresponding latent space vectors to CLIP and
%we build heatmaps in terms of $Con_{spec}$ strength predicates to statistically capture what the model thinks of these inputs
% \nina{This sentence summarizes one of the main contributions. It feels we need a more high-level statement here as an introduction of heatmaps does not seem to be very smooth}\nina{[Suggestion:] Given a group of inputs that are of interest to the user, we use abstract concept-based predicates to analyze how the model reasons about these images. More concretely, we summarize the statistical properties of predicate strengths over this group in the form of a heatmap. Interestingly, such summarization gives powerful insights into understanding the behavior of the group.}\divya{Incorporated.}


% that allows us to scale the analysis to large models. We demonstrate that statistical properties of the strength predicates can be used to obtain insights into understanding model behavior. This aids in exploring the potential of the concept-based analysis of vision models via VLMs paradigm in many more applications

%\susmit{group -> set? ``group" has a formal meaning to it; we don't have operators on this set.}\divya{Addressed.}

Going beyond analyzing model behavior on individual inputs, we apply this approach to statistically analyze the model on collections of inputs.
%Given a set of inputs that are of interest to the user, we use the strength predicates to analyze how the model reasons about these images. More concretely, we summarize the statistical properties of strength predicates over this set in the form of a \emph{heatmap}. 
In particular, given a set of inputs that are of interest to the user (because, for instance, they share their ground-truth labels or predicted labels or are all adversarially perturbed examples), we collect summary statistics about the satisfaction of strength predicates in the form of \emph{heatmaps}. 
Interestingly, such summarization gives powerful insights into understanding the behavior of the model on the input set. For instance, given a set of adversarial inputs, the summarized visualization enabled by the heatmaps can help detect robust/non-robust model features by identifying the concept-based %strength predicates satisfied/violated by the perturbed inputs in comparison with clean inputs. 
strength predicates violated less/more frequently by the perturbed inputs in comparison with the clean inputs. 

%We also present a novel technique that leverages the mapping to VLM to perform fault localization. 
We also present a novel technique that leverages the link between the representation spaces of vision models and VLMs to perform fault localization. 
Given a set of mis-classified images, our %lightweight (\susmit{claim to ``lightweight" is as yet not justified})
approach isolates if the reason for the mis-classification is  due to a bug in the encoder of the vision model or in its classification head. We use  heatmaps to validate the location of bugs and further localize the reasons for failure in terms of the violated strength predicates.


%We describe and demonstrate how we could leverage concept-based heatmaps to aid in applications such as explaining behavior, identifying robust features, and detecting adversarial inputs at runtime. We also present a novel technique to isolate if the reason for a mis-classification is to due a bug in the encoder portion of the vision model or the classification head.


%\divya{Novelty/differences compared to SAIV paper~\cite{mangal2024conceptbased}. Work in progress.}

%Previous work ~\cite{mangal2024conceptbased} demonstrates that if the proxy representation space of the vision model captures accurately the domain semantics (in terms of expert provided concepts), then verification queries for the vision model could be formulated and dispatched using this representation space. In other words, given that the concepts are {\it encoded \it} correctly in the representation space, the verification query checks the functionality of the {\it head \it} on regions of the representation space characterized in terms of the concepts. However, it could happen that while the representation spaces of the vision model and the VLM may be aligned on the set of in-distribution inputs used to build the map, this alignment breaks on other inputs. Such cases are also highlighted in ~\cite{mangal2024conceptbased}; for instance the proxy representation of an image of a plane is closer to a ship, and different from the representation of the same image encoded by the VLM. These cases potentially highlight problems with the encoder of the vision model. As part of this work, we look more closely into this issue, which in turn helps debug the model. Specifically, we find that an overwhelming number of adversarial inputs fall under this category.  Different from ~\cite{mangal2024conceptbased}, we explore the statistical satisfaction of strength predicates, which is more feasible than obtaining proofs. We demonstrate that statistical properties of the strength predicates can be used to obtain insights into understanding model behavior. This aids in exploring the potential of the {\it concept-based analysis of vision models via VLMs paradigm \it} in many more applications.

%\nina{I would not explain to much about 15.}
%\nina{[Suggestion to make the description shorter:] 
%\susmit{I suggest we drop this paragraph and just say, We make the following key contributions in this paper.}
%Previous work ~\cite{mangal2024conceptbased} focuses on the formal verification of strength predicates properties in the representation space. However, it suffers from scalability challenges, especially for large network heads. In this work, we take a statistical approach to analyze neural network behavior in terms of concepts that allows us to scale the analysis to large models. We demonstrate that statistical properties of the strength predicates can be used to obtain insights into understanding model behavior. This aids in exploring the potential of the {\it concept-based analysis of vision models via VLMs paradigm \it} in many more applications.} \divya{Agreed we can drop this para.}

\vspace{0.05in}
\noindent
\textit{\textbf{Contributions.}} Overall, we make the following key contributions in this paper.
%\vspace{-0.5cm}
\begin{itemize}[leftmargin=*]
%\item %We present an approach that enables fine-grained concept-based statistical analysis of vision models to derive useful insights to explain and debug behavior.
%{\it VLM as a Looking Glass. \it} We present a novel approach that analyzes vision models through the lens of VLMs to reason about their behavior in terms of human-understandable concepts.

%provided by experts.
%\susmit{Can drop this if we need to save on space because this is a bit abstract and other contributions support this one.}\divya{Modified. Please check.}
%\item We leverage the work in ~\cite{mangal2024conceptbased} to reason about vision models in a proxy representation space (that of a multi-modal VLM) in terms of predicates that help to formally establish relationship between concepts. We build on this work, to show the potential of this paradigm in useful applications such as isolating the location of bugs in the model, and understanding its behavior on adversarial inputs.

\item {\it VLM-based Semantic Heatmaps. \it} We leverage VLMs to analyze DNNs through  %\textit{concept-based}
\textit{semantic heatmaps} which summarize the statistical evaluation of concept-based strength predicates over a set of inputs in a visual form amenable to analysis. %Specifically, we present three types of heatmaps which help analyse inputs grouped together based on different label-specific categories. 
%Specifically, we present three types of heatmaps which differ based on the sets of inputs considered for analysis.

%We use a case-study of the RIVAL10 dataset and the image classification ResNet18 model to demonstrate the utility of our approach in many applications.

%which facilitate determining if the model makes predictions for the right reasons, identifying problems in the representation space, detecting robustness of model features, and runtime detection of adversarial inputs.

%\item We demonstrate the applications of our approach on the image classification ResNet18 model, on the RIVAL10 dataset.

\item {\it VlM-enabled Offline Analysis. \it} 
\begin{itemize}[leftmargin=*]
    \item {\it Explaining Behavior.\it} %We describe the utility of concept-based heatmaps to examine if model decisions were made for the right reasons. 
    We demonstrate the utility of VLMs and semantic heatmaps to examine if model decisions are made for the right reasons.
%    \divya{Caroline, could you add a sentence highlighting the results of the experiments?} \caroline{I changed describe to demonstrate, I feel that this one is maybe more a demonstration than an experiment?}

    \item {\it Debugging.\it} We present a novel method that leverages VLMs to {\it localize \it} if a wrong classification is due to errors in the {\it encoder \it} or the {\it head \it} of a vision model, and also to give the {\it reasons of failure \it} in terms of the violated predicates. We demonstrate via mutation-based experiments that our technique can successfully isolate errors to encoder or head portions of a model, and also holds potential to perform layer-wise localization.
    
    \item {\it Robustness Analysis of Model Features.\it} We leverage the semantic heatmaps to detect model features that are {\it robust \it} or {\it brittle (non-robust) \it} to adversarial perturbations. Our experiments highlight that a large number of adversarial examples get mis-classified due to encoder errors. Even when the encoder of a model is near accurate for in-distribution inputs, it can have features not robust to adversarial perturbations.
\end{itemize}

\item {\it VLM-enabled Run-time Analysis.\it} We also present a lightweight approach for detecting adversarial inputs at runtime. Using our semantic heatmaps, we are able to achieve about $80\%$ detection accuracy. This shows the potential of semantic heatmaps for efficient runtime analysis.
%We also present a lightweight approach using concept-based heatmaps to detect if an input is adversarial or not at runtime. 
%\divya{Caroline, could you summarize the results for the adversarial detection experiments here?} \caroline{added}

\end{itemize}

%\susmit{Should we refactor contributions into: (a) Semantic Heatmaps (b) Design-time analysis for (b1) explaining model behvaior, (b2) localizing bugs, and (b3) analyzing robustness (c) Runtime monitoring and detection of adversarial perturbations. We can add highlights of experiments for each of these inline with contribution statement.}\divya{Done.}

We see semantic heatmaps as a powerful tool in the toolkit of DNN developers and analysts that can help design new analyses and contribute towards the longer-term goal of safety assurance of DNNs and DNN-enabled systems.
%\divya{Can add a small paragraph summarizing other potential applications, and how the above activities can contribute to the larger goal of safety assurance.}\caroline{I think it's a great idea! this would highlight significance}
%\item Looks into activities such as explaining behavior, localization, adversarial detection, robustness of features so on from the lens of human-understandable concepts. Existing methods typically focus on porting approaches from software engineering of traditional programs which do not make sense for DNNs due to the semantic gap between high level requirements and the implementation. 

%\item Previous work (SAIV) leverages the use of VLMs to create a proxy representation space for vision models.  It demonstrates that if this proxy representation space captures accurately the domain semantics (in terms of expert provided concepts) , then verification queries for the vision model could be formulated and dispatched using this representation space. So basically given that the concepts are "encoded" correctly by the vision model, the verification query checks if the "head" performs the classification correctly.  However, it could happen that the two representation spaces may be aligned for the set of in-distribution inputs used to build the map, but the alignment breaks for other inputs. This is true for cases where the encoder of the vision model does not encode concepts correctly. In such cases, the mapped embedding vector would differ or be far away from the oracle embedding vector (encoded by the VLM for the same input). Specifically, the zero-shot classification ...We found this to be especially true for adversarial inputs, where for a number of the inputs, the representation encoded by the vision model does not match the representation. We explore such cases in this paper, which in turn, helps debug the model.

%\item Statistical analysis (vs verification), helps explores the potential of concept based analysis more - demonstrates more applications.  

%\end{itemize}






%\begin{figure*}
%\centering
%\includegraphics[scale=0.25]{figures/Framework_new.png}
%\caption{Framework: Leveraging VLMs for concept-based analysis of vision models.}
%\label{fig:framework}
%\end{figure*}

%We build on previous work ~\cite{mangal2024conceptbased}, which introduces the logical specification language, $Con_{spec}$ and implements a framework, Fig.~\ref{fig:framework}, that enables the use of VLMs to act as a lens to perform concept-based analysis of other vision models. The language, $Con_{spec}$, enables experts and developers to express domain knowledge as fine-grained logical predicates in terms of human-understandable concepts. The semantics of the language are in terms of the embedding space of VLMs.  The VLM consists of two encoders, one for each modality (text vs. image), that map inputs to the same representation space. The output of the VLM is a {\em similarity score}\footnote{Measured using cosine similarity for CLIP.} between the image and the text. A vision model such as an image classifier can be seen as the composition of an {\em encoder} responsible for translating low-level inputs (pixels composing images) into high-level representations and a {\em head} that makes predictions based on these representations. Reasoning of other vision models in terms of $Con_{spec}$ is enabled by building an affine map between the image embedding space of the vision-based DNN and the corresponding image embedding space of the VLM. As a consequence, the image representation space of a VLM can serve as a proxy for the representation space of a separate vision-based DNN. 

%Fig.~\ref{fig:framework} presents the framework that embodies the idea of leveraging VLMs for concept-based analysis of other vision models. A vision model such as an image classifier (depicted on the left-hand side) can be seen as the composition of an {\em encoder} responsible for translating low-level inputs (pixels composing images) into high-level representations and a {\em head} that makes predictions based on these representations.  The VLM (depicted on the right-hand side), consists of two encoders, one for each modality (text vs. image), that map inputs to the same representation space. The output of the VLM is a {\em similarity score}\footnote{Measured using cosine similarity for CLIP.} between the image and the text. 
%We leverage recent work to build an affine map between the image embedding space of the vision-based DNN and the corresponding image embedding space of the VLM. As a consequence, the image representation space of a VLM can serve as a proxy for the representation space of a separate vision-based DNN.



==> sections/use_cases.tex <==
\section{Applications}
\label{sec:use_cases}

Analysis of semantic heatmaps facilitates a number of analyses that promote better understanding and debugging of vision models. 
In this section, we present the following four applications, and demonstrate them in the context of a case study.

\vspace{0.05in}
\noindent
\textit{\textbf{Explaining Behavior.}} 
%[Corina: this subsection does not provide any useful content: what is the use of the semantic heatmaps precisely? I tried to  re-write]
The first straightforward application is to extract explanations for the model's correct decisions. The explanations are in terms of concept predicates that have high satisfaction probability. This information can help developers to better understand the model's opaque internal logic and can give them confidence that the model understands well the images it processes. This  in turn can help them better assess the generalizability and reliability of the model.

%Testing is typically employed to evaluate model behavior. The set of inputs on which the model produces an output same as the ground-truth, stand to attest the correctness of the model. However, this is insufficient. For instance, a model may classify a set of images correctly as truck. However, unless it can be determined that the model is producing the output label truck for the {\it right reasons \it}, it is not possible to rely on it to classify unseen images of truck  correctly (as the model may have been poisoned to mis-classify many different images to truck). Given a set of inputs correctly classified by a model, we can use semantic heatmaps to {\it explain behavior \it} which helps better assess the generalizability and reliability of the model. %More details are provided in section~\ref{subsec:explain_beh}.




==> sections/use_cases_old.tex <==
\newpage

\section{Use Cases}
\label{sec:use_cases}

\blue{All results regarding ground truth are shown in blue}, \red{All results regarding model output are shown in red}, all heatmaps showing only values $\geq 0.7$.

\green{Differential maps are shown in green}. 

Note: CLIP is not robust to OOD and natural perturbations such as Gaussian Noise or brightness, almost all misclassifications are also misclassified by CLIP.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{heatmaps/no_perturb_correct.png}
    \caption{Rival10 images without any perturbation correctly classified by Resnet18 as truck. y-axis relevant concepts for truck, x-axis not relevant concept for truck. Each grid suggests the proportion of images with relevant $>$ not relevant (through clip). }
    \label{fig:correct_truck}
\end{figure}

\subsection{Debugging/fault localization}
{\bf Divya: As per my understanding there are two types of bug localization we are contributing towards. 
(i) Locating which portion of the network has the bug; comparing the zero-shot classification of g\_enc(x) and g\_enc(map\_(f\_enc(x))). 
(ii) Localizing the features or concept combinations the model is vulnerable to; concept strength predicates based analysis.}


See if checking the heatmaps of different decompositions of encoder and head can give us better localization of the problems. 

Experiments were done with two different decompositions of the encoder and head: 
\begin{enumerate}
    \item Decomp1: 
    \begin{itemize}
        \item ENC: all prediction layers
        \item HEAD: final classification
        \item linear aligner to CLIP: trained with RIVAL10 training data for $50$ epochs using a learning rate of $0.01$, momentum of $0.9$, and weight decay of $0.0005$. Mean Squared Error (MSE) of 0.963 and a Coefficient of Determination (R$^2$) of 0.786 on the test data
    \end{itemize}
    \item Decomp2: 
    \begin{itemize}
        \item ENC: all but the last prediction layer
        \item HEAD: last prediction layer + final classification
        \item linear aligner to CLIP: trained with RIVAL10 training data for $50$ epochs using a learning rate of $0.0001$, momentum of $0.09$, and weight decay of $0.0005$. Mean Squared Error (MSE) of 1.846 and a Coefficient of Determination (R$^2$) of 0.590 on the test data        
    \end{itemize}
\end{enumerate}

\begin{figure*}[t!]
\centering
\captionsetup{justification=centering}
    \begin{tabular}{c c c}
        %\toprule
         %& & & & \\
    
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{heatmaps/targeted_attack_plots/correct_orig_truck1.png}
         \caption{Correctly classified original truck image (aligner of decomp1)}
         \label{fig:cta1}
     \end{subfigure}
     &
     
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{heatmaps/targeted_attack_plots/correct_orig_truck2.png}
         \caption{Correctly classified original truck image (aligner of decomp2)}
         \label{fig:cta2}
     \end{subfigure}
     \\
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{heatmaps/targeted_attack_plots/correct_orig_truck1-th0.5.png}
         \caption{Fig.~\ref{fig:cta1} binarized with threshold 0.5}
         \label{fig:cta1_b}
     \end{subfigure}
     &
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{heatmaps/targeted_attack_plots/correct_orig_truck2-th0.5.png}
         \caption{Fig.~\ref{fig:cta2} binarized with threshold 0.5}
         \label{fig:cta2_b}
     \end{subfigure}
     
     \\
    \end{tabular}
\caption{(fault localization) Comparing aligners trained for decomp1 and decomp2 \red{NEW!}}
\label{fig:adv_detect}
\end{figure*}

Localize fault of Resnet18 facing an adversarial perturbation with two different decompositions, 
see Fig.~\ref{fig:gt_decomp} for results of misclassified images with ground truth truck. see Fig.~\ref{fig:out_decomp} for results of images that are misclassified as trucks.

For Fig.~\ref{fig:gt_decomp} [resp. Fig.~\ref{fig:out_decomp}],

\begin{enumerate}
    \item Fig.~\ref{fig:n1} [resp. Fig.~\ref{fig:o1}] shows ENC error that both decomp1 and decomp2 have, this suggests errors coming from layers decomp1 ENC and decomp2 ENC share
    \item Fig.~\ref{fig:n2} [resp. Fig.~\ref{fig:o2}] shows ENC error that decomp1 has but not decomp2, this should be errors from the extra layer decomp1 ENC has
    \item Fig.~\ref{fig:n3} [resp. Fig.~\ref{fig:o3}] shows ENC error that decomp2 has but not decomp1, since the layers in decomp2 are all in decomp1, it should not have more errors, this would suggest the difference in the linear aligner trained for decomp1 ENC and decomp2 ENC. {\bf Divya: Could it be that the extra layer of decomp1 corrected these errors, but they were mis-classified  by the model due to problems in the head?}
    \item Fig.~\ref{fig:n4} [resp. Fig.~\ref{fig:o4}] shows HEAD error that both decomp1 and decomp2 have, this suggests errors coming from the final layer that decomp1 HEAD and decomp2 HEAD share
    \item Fig.~\ref{fig:n5} and Fig.~\ref{fig:n6} [resp. Fig.~\ref{fig:o5} and Fig.~\ref{fig:o6}] are actually the same as Fig.~\ref{fig:n3} and Fig.~\ref{fig:n2} [resp. Fig.~\ref{fig:o3} and Fig.~\ref{fig:o2}], this is because of how we checked for ENC and HEAD error. We assumed that if it isn't a ENC error, it is a HEAD error. 
\end{enumerate}

%\begin{table}[t]
%    \centering
%    \begin{tabular}{|c|c|c|c|c|}
%    \hline
%    & \multicolumn{2}{|c|}{ground truth truck} & \multicolumn{2}{|c|}{output truck}\\
%    \hline
%    & ENC error & HEAD error & ENC error & HEAD error\\
%    \hline
%       decomp1  &  478 & 14 & 186 & 7\\
%       \hline
%       decomp2  & 468 & 25 & 176 & 21 \\
%       \hline
%    \end{tabular}
%    \caption{Number of errors (these are from two runs so total numbers are slightly different)}
%    \label{tab:my_label}
    
%\end{table}

\begin{figure*}[t!]
\centering
\captionsetup{justification=centering}
    \begin{tabular}{c c c}
        %\toprule
         %& & & & \\
    
     \begin{subfigure}[b]{0.31\textwidth}
         \centering
         \includegraphics[width=\textwidth]{heatmaps/fault/ENC_both_G_0_apgd-ce_fault_decomp_gt_1_MIS.png}
         \caption{ENC error of both decomp1 and decomp2 (455 images)}
         \label{fig:n1}
     \end{subfigure}
     &
     \begin{subfigure}[b]{0.31\textwidth}
         \centering
         \includegraphics[width=\textwidth]{heatmaps/fault/ENC_1not2_G_0_apgd-ce_fault_decomp_gt_1_MIS.png}
         \caption{ENC error of only decomp1 not decomp2 (22 images)}
         \label{fig:n2}
     \end{subfigure}
     &
     \begin{subfigure}[b]{0.31\textwidth}
         \centering
         \includegraphics[width=\textwidth]{heatmaps/fault/ENC_2not1_G_0_apgd-ce_fault_decomp_gt_1_MIS.png}
         \caption{ENC error of only decomp2 not decomp1 (9 images)}
         \label{fig:n3}
     \end{subfigure}
     \\
     \begin{subfigure}[b]{0.31\textwidth}
         \centering
         \includegraphics[width=\textwidth]{heatmaps/fault/HEAD_both_G_0_apgd-ce_fault_decomp_gt_1_MIS.png}
         \caption{HEAD error of both decomp1 and decomp2 (5 images)}
         \label{fig:n4}
     \end{subfigure}
     &
     \begin{subfigure}[b]{0.31\textwidth}
         \centering
         \includegraphics[width=\textwidth]{heatmaps/fault/HEAD_1not2_G_0_apgd-ce_fault_decomp_gt_1_MIS.png}
         \caption{HEAD error of only decomp1 not decomp2 (9 images, same as 2(c))}
         \label{fig:n5}
     \end{subfigure}
     &
     \begin{subfigure}[b]{0.31\textwidth}
         \centering
         \includegraphics[width=\textwidth]{heatmaps/fault/HEAD_2not1_G_0_apgd-ce_fault_decomp_gt_1_MIS.png}
         \caption{HEAD error of only decomp2 not decomp1 (22 images, same as 2(b))}
         \label{fig:n6}
     \end{subfigure}

     \\
    \end{tabular}

\caption{(fault localization) ENC or HEAD error considering all adversarial images with ground truth truck but misclassified as something else.}
\label{fig:gt_decomp}
\end{figure*}


\begin{figure*}[t!]
\centering
\captionsetup{justification=centering}
    \begin{tabular}{c c c}
        %\toprule
         %& & & & \\
    
     \begin{subfigure}[b]{0.31\textwidth}
         \centering
         \includegraphics[width=\textwidth]{heatmaps/fault/ENC_both_O_0_apgd-ce_fault_decomp_o_1_MIS.png}
         \caption{ENC error of both decomp1 and decomp2 (172 images)}
         \label{fig:o1}
     \end{subfigure}
     &
     \begin{subfigure}[b]{0.31\textwidth}
         \centering
         \includegraphics[width=\textwidth]{heatmaps/fault/ENC_1not2_O_0_apgd-ce_fault_decomp_o_1_MIS.png}
         \caption{ENC error of only decomp1 not decomp2 (26 images)}
         \label{fig:o2}
     \end{subfigure}
     &
     \begin{subfigure}[b]{0.31\textwidth}
         \centering
         \includegraphics[width=\textwidth]{heatmaps/fault/ENC_2not1_O_0_apgd-ce_fault_decomp_o_1_MIS.png}
         \caption{ENC error of only decomp2 not decomp1 (4 images)}
         \label{fig:o3}
     \end{subfigure}
     \\
     \begin{subfigure}[b]{0.31\textwidth}
         \centering
         \includegraphics[width=\textwidth]{heatmaps/fault/HEAD_both_O_0_apgd-ce_fault_decomp_o_1_MIS.png}
         \caption{HEAD error of both decomp1 and decomp2 (3 images)}
         \label{fig:o4}
     \end{subfigure}
     &
     \begin{subfigure}[b]{0.31\textwidth}
         \centering
         \includegraphics[width=\textwidth]{heatmaps/fault/HEAD_1not2_O_0_apgd-ce_fault_decomp_o_1_MIS.png}
         \caption{HEAD error of only decomp1 not decomp2 (4 images, same as 2(c))}
         \label{fig:o5}
     \end{subfigure}
     &
     \begin{subfigure}[b]{0.31\textwidth}
         \centering
         \includegraphics[width=\textwidth]{heatmaps/fault/HEAD_2not1_O_0_apgd-ce_fault_decomp_o_1_MIS.png}
         \caption{HEAD error of only decomp2 not decomp1 (26 images, same as 2(b))}
         \label{fig:o6}
     \end{subfigure}

     \\
    \end{tabular}
\caption{(fault localization) ENC or HEAD error considering all adversarial images misclassified as truck.}
\label{fig:out_decomp}
\end{figure*}


\subsection{Detection of robust/non-robust concepts or features}
We compare misclassification facing perturbation with correctly classified non-perturbed images, see which concepts are not affected (are ``robust''), see Fig.~\ref{fig:fea}. The experiments were conducted for both an adversarial perturbation and a natural perturbation, brightness. 

For this use case, we are looking at concepts for images with ground truth truck. Concepts that are preserved for images with and without perturbation can be considered robust. 

\begin{figure*}[t!]
\centering
\captionsetup{justification=centering}
    \begin{tabular}{c c}
        %\toprule
         %& & & & \\
    
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{heatmaps/targeted_attack_plots/adv_gt_truck-th0.5.png}
         \caption{Truck images with adversarial perturbation that are misclassified (threshold 0.5) \red{NEW!}}
         \label{fig:a1}
     \end{subfigure}
     &
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{heatmaps/targeted_attack_plots/orig_adv_truck_gt_diff.png}
         \caption{Diff of Fig.~\ref{fig:a1} with Fig.~\ref{fig:correct_truck} (threshold 0.3) \red{NEW!}}
         \label{fig:a2}
     \end{subfigure}
     \\
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{heatmaps/robust/ALL_G_0_brightness_sev_3_robust_fea_gt.png}
         \caption{Truck images with brightness change that are misclassified}
         \label{fig:b1}
     \end{subfigure}
     &
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{heatmaps/robust/diff_ALL_G_0_brightness_sev_3_robust_fea_gt.png}
         \caption{Diff of Fig.~\ref{fig:b1} with Fig.~\ref{fig:correct_truck}}
         \label{fig:b2}
     \end{subfigure}
     
     \\
    \end{tabular}
\caption{(Detecting robust features) Comparing misclassification of truck images with correct classification of truck images without any perturbation}
\label{fig:fea}
\end{figure*}

\subsection{Adversarial/OOD input detection}
For this one we are only looking at model output, because we won't have ground truth during monitoring. See Fig.~\ref{fig:adv_detect}.

{\bf Divya: For a given label, the set of concept predicates that would be sat Only by the correct-classified inputs, can also help us formulate formal verification checks correctly.}

First, we define a metric IoU to compare two heatmaps. For a single image, the heatmap would be binary, indicating whether this image satisfies  $relevant > not\_relevant$. For a set of images, heatmaps contain proportions of images that have $relevant > not\_relevant$. We binarize the heatmap using a fixed threshold, if value $\geq$ threshold, the value becomes 1, else becomes 0. To compare heatmap of a single image with a heatmap obtained for a set of image, we compute the IoU of the two binarized heatmaps. 

\subsubsection{Using heatmaps to detect adversarial perturbations}

Intuition: for each image that the model output label truck, we check to see if the heatmap for truck-related concepts is closer to the heatmap for all correctly classified non-perturbed truck images (Fig.~\ref{fig:correct_truck}); or closer to the heatmap that the model classifies as truck for adversarially perturbed images (Fig.~\ref{fig:a3}). This is because the model identified the concepts differently for correct truck images and adversarially perturbed images. 

Experiment: 
check to see if comparing heatmap of each image with Fig.~\ref{fig:correct_truck} (no perturb) and Fig.~\ref{fig:a3} (gradient descent cross entropy) can be used to detect whether the images are adversarially perturbed. I also ran a different adversarial perturbation (fab) to see if the type of adversarial attacks would matter.

\red{NEW!}
\red{Results (results updated using heatmaps with more ``balanced'' adv):
Number of images with other gt misclassified as truck: [59 56 59 72 56 45 70 69 67]. Used 80\% original for generating heatmaps and 20\% for testing.
\begin{itemize}
    \item Using diff concepts (any diff concepts)
    \begin{itemize}
        \item Acc on non-perturbed: 0.830
        \item Acc on same attack: 0.205
         \item If we look at particular misclassified images with their ground truth:
        \begin{itemize}
            \item gt 1 car misclassified as truck: 0.017
            \item    gt 2 plane misclassified as truck: 0.179
            \item    gt 3 ship misclassified as truck: 0.085
             \item   gt 4 cat misclassified as truck: 0.931
             \item   gt 5 dog misclassified as truck: 0.875
             \item   gt 6 equine misclassified as truck: 0.756
             \item   gt 7 deer misclassified as truck: 0.786
             \item   gt 8 frog misclassified as truck: 0.681
             \item   gt 9 bird misclassified as truck: 0.821
        \end{itemize}
    \end{itemize}
    \item Using entire heatmap (threshold 0.5)
    \begin{itemize}
        \item Acc on non-perturbed: 0.574
        \item Acc on same attack: 0.437 (NOTE: this is not balanced)
        \item If we look at particular misclassified images with their ground truth:
        \begin{itemize}
            \item gt 1 car misclassified as truck: 0.017
            \item    gt 2 plane misclassified as truck: 0.286
            \item    gt 3 ship misclassified as truck: 0.254
             \item   gt 4 cat misclassified as truck: 0.75
             \item   gt 5 dog misclassified as truck: 0.75
             \item   gt 6 equine misclassified as truck: 0.733
             \item   gt 7 deer misclassified as truck: 0.771
             \item   gt 8 frog misclassified as truck: 0.348
             \item   gt 9 bird misclassified as truck: 0.716
        \end{itemize}
    \end{itemize}
\end{itemize}
}
%\begin{itemize}
%    \item If we use threshold = 0.5 for binarizing the heatmaps
%    \begin{itemize}
%        \item non-perturbed images closer to Fig.~\ref{fig:correct_truck} (correctly detected no adversarial perturbation): 0.729957805907173
%        \item adversarially perturbed images (\textbf{same} type of perturbation) closer to Fig.~\ref{fig:a3} (correctly detected adversarial): 0.7302325581395349
%        \item adversarially perturbed images (\textbf{different} type of perturbation) closer to Fig.~\ref{fig:a3} (correctly detected adversarial): 0.28011611030478956
%    \end{itemize}

%    \item If we use threshold = 0.7 for binarizing the heatmaps
%    \begin{itemize}
%        \item non-perturbed images closer to Fig.~\ref{fig:correct_truck} (correctly detected no adversarial perturbation): 0.9936708860759493
%        \item adversarially perturbed images (\textbf{same} type of perturbation) closer to Fig.~\ref{fig:a3} (correctly detected adversarial): 0.4744186046511628
%        \item adversarially perturbed images (\textbf{different} type of perturbation) closer to Fig.~\ref{fig:a3} (correctly detected adversarial): 0.0420899854862119
%    \end{itemize}
%\end{itemize}


\subsubsection{Airplane images misclassified as truck}

More specifically, looking at airplane images that are misclassified as truck after the adversarial perturbation, see Fig.~\ref{fig:airplane_truck}. Heatmaps in Fig.~\ref{fig:airplane_truck} plot concepts relevant for truck and airplane side by side in the same plot. Truck concepts are marked with a black outline, airplane concepts are marked with an orange outline. 

Our hypothesis is that the heatmap for airplane images misclassified as trucks should have some similarity between correct truck heatmap and correct airplane heatmap. This might give us a way to detect adversarial perturbations. 

\begin{figure*}[t!]
\centering
\captionsetup{justification=centering}
    \begin{tabular}{c c c}
        %\toprule
         %& & & & \\
    
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{heatmaps/targeted_attack_plots/adv_out_truck-th0.5.png}
         \caption{Images with adversarial perturbation that are misclassified as truck (threshold 0.5) \red{NEW!}}
         \label{fig:a3}
     \end{subfigure}
     &
     
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{heatmaps/targeted_attack_plots/adv_out_truck-diffth0.3.png}
         \caption{Diff of Fig.~\ref{fig:a3} with Fig.~\ref{fig:correct_truck} (threshold 0.3) \red{NEW!}}
         \label{fig:a4}
     \end{subfigure}
     \\
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{heatmaps/detection/ALL_O_0_brightness_sev_3_detection_o.png}
         \caption{Images with brightness change that are misclassified as truck}
         \label{fig:b3}
     \end{subfigure}
     &
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{heatmaps/detection/diff_ALL_O_0_brightness_sev_3_detection_o.png}
         \caption{Diff of Fig.~\ref{fig:b3} with Fig.~\ref{fig:correct_truck}}
         \label{fig:b4}
     \end{subfigure}
     
     \\
    \end{tabular}
\caption{(Detecting adversarial/OOD perturbation) Comparing images classified as truck with correctly classified truck images with no perturbation}
\label{fig:adv_detect}
\end{figure*}



\begin{figure*}[t!]
\centering
\captionsetup{justification=centering}
    \begin{tabular}{c c}
        %\toprule
         %& & & & \\
    
     \begin{subfigure}[b]{0.4\textwidth}
         \centering
         \includegraphics[width=\textwidth]{heatmaps/targeted_attack_plots/bird_misclassified_as_truck-th0.5.png}
         \caption{Bird misclassified as truck}
         \label{fig:at1}
     \end{subfigure}
     &
     \begin{subfigure}[b]{0.4\textwidth}
         \centering
         \includegraphics[width=\textwidth]{heatmaps/targeted_attack_plots/truck_misclassified_as_bird-th0.5.png}
         \caption{Truck misclassified as bird}
         \label{fig:at1}
     \end{subfigure}
     \\
     
     \begin{subfigure}[b]{0.4\textwidth}
         \centering
         \includegraphics[width=\textwidth]{heatmaps/targeted_attack_plots/correct_truck-th0.5.png}
         \caption{Non-perturbed images correctly classified as truck}
         \label{fig:at2}
     \end{subfigure}
     &
     \begin{subfigure}[b]{0.4\textwidth}
         \centering
         \includegraphics[width=\textwidth]{heatmaps/targeted_attack_plots/correct_bird-th0.5.png}
         \caption{Non-perturbed images correctly classified as bird}
         \label{fig:at3}
     \end{subfigure}
     
    \end{tabular}
\caption{(Detecting adversarial/OOD perturbation) Specifically looking at bird images misclassified as truck after adversarial perturbations. Comparing this with concepts relevant for both truck (indicated by red outline) and bird (indicated by blue outline). With 20 images each. \red{NEW!}}
\label{fig:airplane_truck}
\end{figure*}

